Robust Estimation for Random Graphs

We study the problem of robustly estimating the parameter $p$ of an Erd\H{o}s-R\'enyi random graph on $n$ nodes, where a $\gamma$ fraction of nodes may be adversarially corrupted. After showing the deficiencies of canonical estimators, we design a computationally-efficient spectral algorithm which estimates $p$ up to accuracy $\tilde O(\sqrt{p(1-p)}/n + \gamma\sqrt{p(1-p)} /\sqrt{n}+ \gamma/n)$ for $\gamma < 1/60$. Furthermore, we give an inefficient algorithm with similar accuracy for all $\gamma <1/2$, the information-theoretic limit. Finally, we prove a nearly-matching statistical lower bound, showing that the error of our algorithms is optimal up to logarithmic factors.

==> Reg-graphs.tex <==


In this subsection we derive some simple consequences of regularity of the graph that we will use subsequently in establishing the guarantees for our algorithms.
One of these consequences is a simple inefficient algorithm to recover a crude estimate of $p$ that has an optimal dependence on all parameters other than $\regpar$.

For a subset $S\subseteq[n]$ and adjacency matrix $A$, we will use \tcr{$p_S:= \frac{\sum_{i,j \in S} A_{i,j}}{|S|^2}$} to denote the empirical fraction of edges present in the subgraph induced by a set $S$.


The following lemma lists some simple but useful consequences of the regularity conditions that we make use in the later proofs.
\begin{lemma}
Suppose $0\le \regpar_1,\regpar_2< 1/2$ and adjacency matrix $\AdjM$ has a node subset  $\goodnodes\subseteq [n] $ that satisfies $(\regpar_1,\regpar_2,p)$-regularity, then 
\begin{enumerate}
 \item For all $\goodnodesub\subseteq \goodnodes $,
 \begin{align}\label{eq:llemc}
     \|(\AdjM - p_{\goodnodesub})_{\goodnodesub\times \goodnodesub}\|\le 2n\cdot \Boundb(p,n).
\end{align}
%and 
%\begin{align}\label{eq:llema}
%    |\goodnodesub|\cdot |x-p | -n\cdot \Boundb(p,n) \le \|(\AdjM - x)_{\goodnodesub\times \goodnodesub}\|\le  |\goodnodesub|\cdot |x-p| +n\cdot \Boundb(p,n),
%\end{align}
 \item For all $\goodnodesub\subseteq \goodnodes $ of size $\ge (1-\regpar_2)n$,
\begin{align}\label{eq:llemb}
|p_{\goodnodesub}-p|\le {4 \Bounda(\regpar_2,p,n)}.
\end{align}
\end{enumerate}
\end{lemma}
\begin{proof}
%Equation~\eqref{eq:llema} follows from regularity condition~\ref{pt:first-point} and triangle inequality.
%Next 
First we prove Equation~\eqref{eq:llemc}. From triangle inequality
\[
 \|(\AdjM - p_{\goodnodesub})_{\goodnodesub\times \goodnodesub}\| \le  \|(\AdjM - p)_{\goodnodesub\times \goodnodesub}\|+|p - p_{\goodnodesub}|\cdot {\goodnodesub}.
\]
From Lemma~\ref{lem:specnormlb} we have
\[
\|(\AdjM - p)_{\goodnodesub\times \goodnodesub}\|\ge |\goodnodesub|\cdot|p_{\goodnodesub}-p| .
\]
Combining the above two equations proves Equation~\eqref{eq:llemc},
\[
\|(\AdjM - p_{\goodnodesub})_{\goodnodesub\times \goodnodesub}\| \le 2\|(\AdjM - p)_{\goodnodesub\times \goodnodesub}\|\le 2n\cdot \Boundb(p,n),
\]
where the last inequality follows from regularity condition~\ref{pt:first-point}.

Next, Equation~\eqref{eq:llemb} is obtained by using $\goodnodesub=\goodnodesubanother$ in regularity condition~\ref{pt:second-point} and $|\goodnodesub|\ge n/2$.
\end{proof}

%Equation~\eqref{eq:llema} in the lemma implies that if adjacency matrix of any subset of good nodes is centered around $x$ that is far from $p$, then it will have a large spectral norm and vice versa.
Equation~\eqref{eq:llemc} implies that if adjacency matrix of any subset of good nodes is centered around its empirical fraction of the edges, then its spectral norm is bounded.

Equation~\eqref{eq:llemb} implies that for any subset of good nodes that excludes at most $\regpar_2n$ nodes, the empirical fraction of the edges in subgraph induced by it estimates $p$ accurately. 





The next theorem shows that if for any subset $S\subseteq[n]$ of size $\ge n/2$ nodes, the spectral norm of its submatrix centered with respect to $p_S$ is small then $p_S$ is a reasonable estimate of $p$.
\begin{theorem}\label{th:newth}
Suppose $0\le \regpar_1,\regpar_2< 1/2$ and adjacency matrix $\AdjM$ has node subset  $\goodnodes\subseteq [n] $ that satisfy $(\regpar_1,\regpar_2,p)$-regularity, then for all $S\subseteq [n]$ such that $|S|\ge n/2$, we have 
\[
 |p_{S}-p|\le \frac{\|(\AdjM - p_{S})_{S\times S} \|+n\cdot \Boundb(p,n)}{(1/2-\regpar_1)n }.
\]
\end{theorem}
\begin{proof}
From triangle inequality,
\[
\|(\AdjM - p_{S})_{(S\cap \goodnodes)\times (S\cap \goodnodes)} \| \ge |(p- p_{S})\cdot(S\cap \goodnodes)|-\|(\AdjM - p)_{(S\cap \goodnodes)\times (S\cap \goodnodes)} \|.
\]
Then using Lemma~\ref{lem:spsubmat}
\[
|(p- p_{S})\cdot(S\cap \goodnodes)|\le \|(\AdjM - p_{S})_{(S\cap \goodnodes)\times (S\cap \goodnodes)} \| +\|(\AdjM - p)_{(S\cap \goodnodes)\times (S\cap \goodnodes)} \|\le  \|(\AdjM - p_{S})_{S\times S} \| +\|(\AdjM - p)_{ \goodnodes\times \goodnodes} \|.
\]
Finally, noting that $|S\cap \goodnodes|\ge |S|-|\goodnodes^c|\ge |S|-\regpar_1 n\ge n/2-\regpar_1 n$ proves the theorem.
\end{proof}


\begin{theorem}\label{th:ineff}
Suppose $0\le \regpar_1,\regpar_2< 1/2$ and adjacency matrix $\AdjM$ has node subset  $\goodnodes\subseteq [n] $ that satisfy $(\regpar_1,\regpar_2,p)$-regularity. Let
\[\hat S \gets \arg\min_{S\subseteq [n]:|S|\ge n/2}\|(\AdjM - p_{S})_{S\times S} \|, \]
then 
\[
 |p_{\hat S}-p|\le \frac{3}{(1/2-\regpar_1) }\cdot \Boundb(p,n).\]
\end{theorem}
\begin{proof}
From the definition of $\hat S$,
\[\|(\AdjM - p_{\hat S})_{\hat S\times \hat S} \|\le \|(\AdjM - p_{\goodnodes})_{\goodnodes\times \goodnodes} \|\le2n\cdot \Boundb(p,n), 
\]
where the last inequality uses Equation~\eqref{eq:llemc}. Then the proof follows from Theorem~\ref{th:newth}
\end{proof}

Note that the set $\hat S$ can be found by iterating over all subsets of $[n]$. This gives us a simple algorithm to estimate $p$.
However, there are two disadvantages. First, the algorithm has a running time exponential in $n$. Second it gives us sub-optimal bound for small $\regpar_1$.

%In the next subsection we derive an efficient algorithm to find a subset $S^*$ such that $\|(\AdjM - p_{S^*})_{S^*\times S^*} \| \le  \mathcal O(n\cdot \Boundb(p,n))$. For $\regpar_1 < 0.49?$, this will imply estimation up to an accuracy of $\mathcal O( \Boundb(p,n))$.



\iffalse
\begin{algorithm}[H]
  \begin{algorithmic}
    \Require{corruption parameter $\corr\in [1/{n}, 1/2)$, adjacency matrix $A$}
    \State{$\hat S \gets \arg\min_{S\subseteq [n]:|S|\ge n/2+1}\|(\AdjM - p_{S})_{S\times S} \| $}\\
    \Return $\hat S$ 
  \end{algorithmic}
  \caption{\label{algo:ineff}Inefficient algorithm for estimating $p$}
\end{algorithm}
\fi

==> concentration-properties.tex <==
Non-trivial robust estimation is only possible since uncorrupted Erd\H{o}s-R\'enyi random graphs enjoy a rich structure.
In this section, we establish concentration results that capture the structure which our algorithms will exploit.

Recall that $\tilde A$ and $A$ are the adjacency matrix of the uncorrupted and the corrupted graphs, respectively.
For notational convenience, we will use \tcr{$p_S:= \frac{\sum_{i,j \in S} A_{i,j}}{|S|^2}$} as the empirical fraction of edges present in the subgraph induced by a set $S \subseteq [n]$.
Note that this is defined in terms of $A$ (rather than $\tilde A$) as our algorithms will only have access to $A$.

Furthermore, we define the following quantity $\kappa$, which we use in the bounds of several quantities.
For $\alpha\in (0,1]$, $p\in [0,1]$ and $n> 0$, let 
\begin{align}
\kappa(\alpha,p,n) := \max\Bigg(\sqrt{\frac{p}{n}\ln\frac{e}{\alpha}+\frac{\ln n}{n^2}} ,\frac{1}{n}\ln\frac{e}{\alpha}\Bigg).\label{eqn:def-alpha}
\end{align}
Note that for any fixed $p$ and $n$, $\kappa(\alpha,p,n)$ is a decreasing function of $\alpha$.



% \begin{lemma}[Chernoff bound]
% Let $X_1,X_2,...,X_t\sim \text{Ber}\,(p)$ be $t$ independent Bernoulli random variables. Then for any $\lambda>0$
% % \[
% % \Pr\big[\big|\sum X_i-tp\big|\ge tp\delta \big]\le 2\exp\Paren{-\frac{\delta^2 t p}{2+\delta}}\le 2\exp\Paren{-\min\Paren{\frac{\delta^2 t p}{3},\frac{\delta t p}{3}}}.
% % \]
% % Alternately, we can write, 
% \begin{align}
% \Pr\big[\big|\sum^t_{i=1} X_i-tp\big|\ge \lambda \big]\le 2\exp\Paren{-\min\Paren{\frac{\lambda^2}{3tp},\frac{\lambda}{3}}}.
% \label{eqn:chernoff}    
% \end{align}
% \end{lemma}

\tcr{We now show that empirical means of all sufficiently large submatrices of $\tilde A$ simultaneously concentrate around $p$. The proof follows a Chernoff and union bound style argument, and is provided in Section~\ref{sec:app-mainconth}.}

\begin{theorem}\label{th:mainconth} 
Let $\tilde A$ be the adjacency matrix of a sample from $G(n,p)$. 
With probability at least $1-3 n^{-2}$, simultaneously for all $\alpha\in[\frac{1}{ \sqrt n},\frac{1}{2}]$, we have
%and $S, S'\subseteq [n]$ such that 
%\[
%|S|, |S'|\in [0, \alpha n]\cup [n-\alpha n, n]
%\]
%we have
\[
\max_{|S|,|S'|\in \setsize_\alpha}\Bigg|{\sum_{i\in S,\,j\in S'}(\tilde A_{i,j}-p)}\Bigg|\le 4\max\Big\{ 16\alpha n\sqrt{{p n}\ln\frac{e}{\alpha }},60\alpha n\ln\frac{e}{\alpha }\Big\},
\]
where we define $\setsize_{\alpha}:= [0, \alpha n]\cup [n-\alpha n, n]$.
\end{theorem}
\iffalse
\begin{theorem}\label{th:mainconth}(alternative to above) With probability at least $1-3 n^{-2}$, simultaneously for all \tcr{$\alpha\in[\frac{1}{ \sqrt n},\frac{1}{2}]$} and for all $S,S'\subseteq[n]$ with $|S|,|S'|\in [0, \alpha n]\cup [n-\alpha n, n]$,  we have
%and $S, S'\subseteq [n]$ such that 
%\[
%|S|, |S'|\in [0, \alpha n]\cup [n-\alpha n, n]
%\]
%we have
\[
\Bigg|{\sum_{i\in S,\,j\in S'}(\tilde A_{i,j}-p)}\Bigg|\le 4\max\Big\{ 16\alpha n\sqrt{{p(1-p)n}\ln\frac{e}{\alpha }},60\alpha n\ln\frac{e}{\alpha }\Big\}.
\]
\end{theorem}
\fi
The following corollary describes the main concentration results that our algorithms depend on.
In the remaining subsections describing our algorithm, we will condition on these results.

%we state the results on concentration of spectral norms and empirical means of the adjacency matrices that we will use in the following sections. 
% The next corollary follows from the above theorem, Lemma~\ref{lem:goodspecnormnew} and Lemma~\ref{lem:spsubmat}.

\begin{corollary}\label{cor:goodspecnorm} 
For any $\corr \in [0,1]$, let $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$. 
Recall that $\goodnodes$ is the set of uncorrupted nodes. 
There exist universal constants $c$ and $c_1$ such that 
for \tcr{any} $n,p$, with probability at least $1-4n^{-2}$, 
\begin{enumerate}
    \item \label{pt:first-point} For all $\goodnodesub\subseteq \goodnodes $, 
    \[ \|(A - p)_{\goodnodesub\times \goodnodesub}\| \le  c\sqrt{np+\ln n}\le c n\min_{\alpha\in(0,1]}\kappa(\alpha,p,n). \]
   \item   \label{pt:second-point} For all $\alpha\in[\frac{1}{\sqrt n},\frac{1}{2}]$ and all $\goodnodesub , \goodnodesubanother\subseteq \goodnodes $ such that $|\goodnodesub |,|\goodnodesubanother|\in [0, \alpha n]\cup [n-\alpha n, n]$, then
\[
\Bigg|{\sum_{i\in \goodnodesub }\sum_{j\in \goodnodesubanother}(A_{i,j}-p)}\Bigg|\le  c_1\alpha n^2\cdot\kappa(\alpha,p,n). 
\]
\item  \label{pt:third-point}
 For all $\alpha\in[\frac{1}{\sqrt n}, \frac12]$ and all $\goodnodesub \subseteq \goodnodes $ with $|\goodnodesub |>n-\alpha n$, 
\begin{equation}\label{eq:usefula}
|p_{\goodnodesub }-p|\le 4c_1\alpha \cdot\kappa(\alpha,p,n).
\end{equation}
\end{enumerate}
\end{corollary}

\begin{proof}
Recall that $\tilde A$ is the adjacency matrix of the original graph $G\sim G(n,p)$. 
We use the following bound on the spectral norm of a centered version of $\tilde A$, which follows from Remark 3.13 of~\cite{BandeiraVH16}. 
\begin{lemma}\label{lem:goodspecnormnew}
There exist a universal constant $c$ such that with probability at least $1-n^{-2}$,
$\norm{\tilde A - p} \le c\sqrt{np+\ln n}$.  
\end{lemma}
To establish the first property, note that $A$ and $\tilde A$ agree on $(i,j)\in \goodnodes \times \goodnodes $, and therefore by Lemma~\ref{lem:spsubmat} and Lemma~\ref{lem:goodspecnormnew}, $\|(A - p)_{\goodnodesub \times \goodnodesub }\| = \|(\tilde A - p)_{\goodnodesub \times \goodnodesub }\| \le \|(\tilde A - p)\|\le c\sqrt{np+\ln n} $.
The second property is a restatement of Theorem~\ref{th:mainconth}.
The last property can be obtained by plugging $\goodnodesub =\goodnodesubanother$ into the second property.
\end{proof}

We will also need the following simple concentration bound, which will be useful when handling the case when the graph is very sparse.
\begin{theorem}
  \label{thm:extreme-conc}
  Let $G$ be a sample from $G(n,p)$, where $p \leq \frac{1}{n-1}$. 
  Every node in $G$ has degree at most $1 + 9 \log n$ with probability at least $1 - 2n^{-2}$.
\end{theorem}
\begin{proof}
  Let the degree of node $i$ be denoted by $Z_i \sim \Bin(n-1,p)$.
  We apply the Chernoff bound (Lemma~\ref{lem:chernoff}) on $Z_i$, to find the probability that node $i$ has degree greater than $1 + \beta \log n$, where $\beta \geq 3$ is any constant.
  %\[\Pr\left[Z_i \geq (n-1)p + \beta \log n \right] \leq \exp\left(-\dkl\left(p + \frac{\beta \log n }{n-1} || p\right) n\right) \leq \exp\left(-\frac{\beta^2 \log^2 n}{(n-1)^2} n\right)\]
  \begin{align*}
    \Pr\left[Z_i \geq 1 + \beta \log n\right] &\leq \Pr\left[Z_i \geq (n-1)p + \beta \log n \right] \\
    &\leq 2\exp\left(- \min\left\{\frac{\beta^2 \log^2 n}{3(n-1)p}, \frac{\beta \log n}{3}\right\} \right) \\
    &\leq 2\exp\left(-  \frac{\beta \log n}{3}\right) \\
    &= 2 n^{-\beta/3}
  \end{align*}
The proof concludes by applying the union bound to all $n$ nodes and setting $\beta = 9$.
\end{proof}



\subsubsection{Implications of Concentration}

Item~\ref{pt:first-point} of Corollary~\ref{cor:goodspecnorm} bounds the spectral norm when the adjacency matrix is centered around the true edge parameter $p$. 
However, since $p$ is unknown to the algorithm, it will only be able to compute the spectral norm of a submatrix centered with respect to its empirical edge parameter.
We bound this quantity for all sufficiently large submatrices \tcr{of uncorrupted nodes}.
%The following lemma bounds the spectral norm of sufficiently large mean-centered submatrices that are subsets of the uncorrupted nodes $\goodnodes $.
\begin{lemma}\label{lem:tobenamed}
For any $\corr \in [\frac{1}{\sqrt{n}}, \frac{1}{20}]$, let $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$. 
Suppose the events in Corollary~\ref{cor:goodspecnorm} hold.
%For any matrix $A\in \mathbb R^{n\times n}$, $\gamma\in [\frac{1}{\sqrt{n}}, \frac{1}{20}]$ and
%For all $\goodnodesub \subseteq \goodnodes $ of size $|\goodnodesub |\ge (1-10\gamma)n$ and the events in Corollary~\ref{cor:goodspecnorm} holds for $\alpha=10\gamma$. 
Then simultaneously for all $\goodnodesub \subseteq \goodnodes $ of size $|\goodnodesub |\ge (1-10\gamma)n$, for some constant $c_2$, we have
\[
\|(A-p_{\goodnodesub })_{\goodnodesub \times \goodnodesub }\|\le  c_2n \cdot \kappa(10\gamma,p,n).
\]
\end{lemma}
\begin{proof}
By Lemma~\ref{lem:triangleineq}, we have
\begin{align*}
 \|(A-p_{\goodnodesub })_{\goodnodesub \times \goodnodesub }\|= \|(A-p+p-p_{\goodnodesub })_{{\goodnodesub }\times{\goodnodesub }}\|
 \le  \|(A-p)_{{\goodnodesub }\times{\goodnodesub }}\|+ |p-p_{\goodnodesub }|\cdot|{\goodnodesub }|.
\end{align*}

By Item~\ref{pt:third-point} of Corollary~\ref{cor:goodspecnorm} with $\alpha=10\gamma$, we have $|p-p_{\goodnodesub }|\cdot|{\goodnodesub }|\le 40 \gamma  c_1 \cdot\kappa(10\gamma,p,n) \cdot n$.

By Item~\ref{pt:first-point} of Corollary~\ref{cor:goodspecnorm} with $\alpha=10\gamma$, we get $\|(A-p)_{{\goodnodesub }\times{\goodnodesub }}\|\le cn \cdot\kappa(10\gamma,p,n) \cdot n$.

Finally, observing that  $40\gamma\le 2$ and then letting $c_2 := c+2c_1$ proves the lemma.
\end{proof}

%\tcr{The previous lemma holds only for subsets of $\goodnodes $. We will not have access to $\goodnodes $, and the next lemma bounds the spectral norm of the submatrix 
% $(A-p_S)_{(S\cap \goodnodes )\times(S\cap \goodnodes )}$ in terms of $|p_{S\cap \goodnodes }-p_S|$, \newhz{which is} the difference in the empirical means of $A$ restricted to ${S\times S}$ and ${(S\cap \goodnodes)  \times (S\cap \goodnodes) }$.}
 
 The preceding lemma holds only for submatrices corresponding to sets $S$ which are purely subsets of the uncorrupted nodes $\goodnodes$.
 Our algorithm is unlikely to identify such $S$, and will instead interact with sets $S$ such that $S \cap \goodnodes$ and $S \cap \bad$ are both non-empty.
 Specifically, our algorithm will measure the spectral norm of matrices $(A-p_S)_{S \times S}$.
 The following lemma upper bounds how much the submatrix corresponding to the indices $S \cap \goodnodes$ can contribute to this quantity.
 As we will establish later, this implies that if the spectral norm of $(A-p_S)_{S \times S}$ is large, then it must be because the contribution from $S \cap \bad$ is large, a property which our algorithm will exploit.
 \gnote{Is the above paragraph true?}
 
\begin{lemma}\label{lem:justnamed}
For any $\corr \in [\frac{1}{\sqrt{n}}, \frac{1}{20}]$, let $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$. 
Suppose the events in Corollary~\ref{cor:goodspecnorm} hold.
Then simultaneously for all sets $S \subseteq [n]$ of size $|S |\ge (1-9\corr)n$, for some constant $c_2$, we have
\[
\|(A-p_S)_{(S\cap \goodnodes )\times(S\cap \goodnodes )}\|\le  c_2n \cdot \kappa(10\gamma,p,n)+|S\cap \goodnodes |\cdot|p_{S\cap \goodnodes }-p_S|.
\]
\end{lemma}
\begin{proof}
Note that $S\cap \goodnodes \subseteq \goodnodes $. 
\begin{align*}
 \|(A-p_S)_{(S\cap \goodnodes )\times(S\cap \goodnodes )}\|&= \|(A-p_{S\cap \goodnodes }+p_{S\cap \goodnodes }-p_S)_{(S\cap \goodnodes )\times(S\cap \goodnodes )}\|\\
 &\le  \|(A-p_{S\cap \goodnodes })_{(S\cap \goodnodes )\times(S\cap \goodnodes )}\|+ |p_{S\cap \goodnodes }-p_S|\cdot|S\cap \goodnodes |\\
 &\le   c_2n \cdot \kappa(10\gamma,p,n)+ {|p_{S\cap \goodnodes }-p_S|\cdot|S\cap \goodnodes |},
 %\\ %\frac{|\sum_{i,j\in S\cap \goodnodes }(A_{i,j}-p_S)|}{|S\cap \goodnodes |^2}\cdot|S\cap \goodnodes |\\
% &=   c_2n \cdot \kappa(10\gamma,p,n)+ |S\cap \goodnodes |\cdot|p_{S\cap \goodnodes }-p_S|,
\end{align*}
here the last inequality follows from Lemma~\ref{lem:tobenamed} as  and $|S\cap \goodnodes |\ge |S|-|B|=|S|-\gamma n\ge (1-10\gamma)n$.
\end{proof}



% \begin{proof}
% Since $M$ is a symmetric matrix we know that for the top eigenvector $v\in \mathbb R^n$ and for some $\lambda\in \mathbb R$  we have  $M v = \lambda v $ and $\|M\| = |\lambda|$. 
% Then
% \begin{align*}
% \|M_{S\times [n]}\, v\|^2= \|\lambda v_{S}\|^2 = \|v_{S}\|^2\cdot \lambda^2= (\|v\|^2-\|v_{[n]\setminus S}\|^2)\cdot \lambda^2=(1-\|v_{[n]\setminus S}\|^2)\cdot \lambda^2.    
% \end{align*}
% Next,
% \begin{align*}
% \|M_{S\times [n]} \,v\|^2 &= \|(M_{S\times S}+M_{S\times [n]\setminus S}) v\|^2\\
% &= \|M_{S\times S}\, v_S+M_{S\times [n]\setminus S} \,v_{[n]\setminus S}\|^2\\
% &\le{ 2\|M_{S\times S}\, v_S\|^2+2\|M_{S\times [n]\setminus S} \,v_{[n]\setminus S}\|^2}\\
% &\le 2\|M_{S\times S}\|^2+ 2\|v_{[n]\setminus S}\|^2\cdot \|M_{S\times [n]\setminus S}\|^2\\
% &\le 2\alpha^2\|M\|^2+ 2\|v_{[n]\setminus S}\|^2\cdot \|M\|^2\\
% &=  2\alpha^2\lambda^2+ 2\|v_{[n]\setminus S}\|^2\cdot \lambda^2,
% \end{align*}
% {where the last inequality uses Lemma~\ref{lem:spsubmat}.}



% Combining the two bounds proves the result.
% \end{proof}


==> lower-bound.tex <==
\def \derg {DG}
In this section, we prove our main lower bound for robust parameter estimation in Erd\H{o}s-R\'enyi random graphs.
This implies that our algorithms are tight up to logarithmic factors.

\begin{theorem}
\label{thm:lower-bound}
%Let $\corr>1/\sqrt{\ns}$ and $p<0.5$. 
Let $p\leq0.5$. Then there exists a $\corr$-oblivious adversary such that no algorithm can distinguish between $G(n,p)$ and $ G\Paren{n,p+0.1\max\Paren{\corr\sqrt{p/n},  \gamma/\ns,  \sqrt{p}/n}}$ with probability at least 0.8.
%\tcr{no algorithm that distinguishes between $G(n,p)$ and $ G\Paren{n,p+0.1\max\Paren{\corr\sqrt{p/n},  \gamma/\ns,  \sqrt{p}/n}}$ has probability of probability of success $\ge$0.8.}
\end{theorem}
By symmetry, a similar statement holds for $p > 0.5$, with $p$ replaced by $1-p$. 
Combining these two statements gives the lower bound in Theorem~\ref{thm:lower-bound-main}.

To derive our lower bounds, we will consider a directed variant of the Erd\H{o}s-R\'enyi random graph model.

\begin{definition}[Directed Erd\H{o}s-R\'enyi graphs]
 \label{def:bi-gnp}
 The directed Erd\H{o}s-R\'enyi random graph model on $n$ nodes with parameter $p$, denoted as  $\derg (\ns, p)$, is the distribution over directed graphs on $n$ nodes where each edge is present with probability $p$, independently of the other edges. 
\end{definition}
We note the following equivalent method of sampling from  this model.
\begin{claim}
One can sample from $\derg(\ns, p)$ via the following process.
For each node $u$, draw the node's degree $d$ from the distribution $\Bin(n-1, p)$.
Then add edges from $u$ to all nodes in a randomly selected subset of the other nodes of size $d$.
\end{claim}

We will show a reduction from $\gamma$-corrupted parameter estimation in the directed Erd\H{o}s-R\'enyi model to the standard one, indicating that the latter is no easier.
We will then prove a lower bound for this setting will imply lower bounds for the standard Erd\H{o}s-R\'enyi model.

\begin{lemma}
\label{lem:undirected_to_directed}
Suppose there exists an algorithm for estimating $p$ in $G(n,p)$ under $\corr$-corruptions.
Then there exists an algorithm for estimating $p$ in $\derg(n, p)$ under $\corr$-corruptions with less or equal error.
\end{lemma}
\begin{proof}
We prove this lemma by converting a $\corr$-corrupted graph from $\derg(n,p)$ to a $\corr$-corrupted graph from $G(n,p)$.
Then one can run the algorithm for the undirected setting to obtain an estimate of $p$, which implies the same error guarantees for the directed instance.

Suppose there exists a random directed graph $\derg\sim \derg(n,p)$ which is $\corr$-corrupted by an adversary.
Assume there exists some lexicographic ordering of the nodes (e.g., they are numbered from $1$ to $n$).
We define a corresponding undirected graph $G$ as follows: let there be an edge between nodes $i$ and $j$ in $G$ if there exists an edge from $i$ to $j$ in $DG$ and $i<j$. Sans corruptions, this converts $\derg(n,p)$ into $G(n,p)$ since the edges are still independent and the probability of each edge existing is $p$. Furthermore, when at most $\corr n$ nodes in the original directed graph are modified, at most $\corr n$ nodes are changed in the corresponding undirected graph. 
\end{proof}


For the remainder of this section, we prove an analogue of Theorem~\ref{thm:lower-bound} for directed Erd\H{o}s-R\'enyi graphs.
A subsequent application of Lemma~\ref{lem:undirected_to_directed} will imply Theorem~\ref{thm:lower-bound}.

We start with the first term in the max in Theorem~\ref{thm:lower-bound}.
%We will need the following lemma in the proof of Theorem~\ref{thm:lower-bound}. 
The following lemma is similar to Lemma 4 of~\cite{QiaoV18}, though we employ a more careful analysis with respect to $p$.
Roughly speaking, it says that two binomial distributions with similar parameters can be lightly mixed with other distributions such that the resulting mixtures are equal.
Observe that we consider distributions over $\newhz{[n-1]}$ -- this will be applied to the outdegree distribution of nodes in our directed random graphs.


\begin{lemma}
\label{lem:same_distribution}
Let $\corr<0.5$, $p<0.5$, $q=p+0.1\corr\sqrt{p/n}$ and $n\geq10$. There exists two distributions $P_y$ and $Q_y$ over $\{0,1\}^{\ns-1}$ such that
\[
\left(1-\frac{\gamma}{2}\right)P_x + \frac{\gamma}{2} P_y = \left(1-\frac{\gamma}{2}\right)Q_x + \frac{\gamma}{2} Q_y,
\]
%where $P_x = \Bin (\newhz{n-1},p)$, and $Q_x = \Bin (\newhz{n-1},q)$.
where \newhz{$P_x = \Ber(p)^{\otimes n-1}$, and $Q_x = \Ber(q)^{\otimes n-1}$}.
\end{lemma}

\begin{proof}
We first bound the total variation distance between $P_x$ and $Q_x$.
Note that \newhz{this distance is the same with the total variation distance between $\Bin (n-1,p)$ and $\Bin (n-1,q)$, which can be bounded} as~\cite{Roos03a},~\cite[Eq (2.16)]{AdellJ06}.
% \begin{align*}
% d_{\rm TV}\left(\Bin (n,p),\Bin (n,p+x) \right)
% &\le \sqrt{\frac e2} \frac{\tau(x)}{(1-\tau(x))^2},
% \end{align*}
% where 
% $\tau(x)= x\cdot \sqrt{\frac{n+2}{2p(1-p)}}$. In our case, $x=0.1\corr\sqrt{p/n}$, and 
\begin{align*}
d_{\rm TV}\left(\Bin (n-1,p),\Bin (n-1,p+x) \right)
&\le \sqrt{\frac e2} \frac{\tau(x)}{(1-\tau(x))^2},
\end{align*}
where 
$\tau(x)= x\cdot \sqrt{\frac{n+1}{2p(1-p)}}$. In our case, $x=0.1\corr\sqrt{p/n}$, and 
\begin{align*}
\tau(x) = 0.1\corr\sqrt{\frac pn}\sqrt{\frac{n+1}{2p(1-p)}}
 \le 0.1 \cdot 1.1 \corr = 0.11\corr.
\end{align*}
Therefore,
\begin{align}
\label{equ:tvdistance}
d_{\rm TV}\left(P_x, Q_x\right) \le 0.15\corr. 
\end{align}

    We now describe how to construct $P_y$ and $Q_y$ over $\{0,1\}^{n-1}$. 
    Let $Z$ be a vector of length $2^{n-1}$ indexed by vectors in $\{0,1\}^{n-1}$, where for $w\in\{0,1\}^{n-1}$, $Z_w = \max (P_x(w), Q_x(w))$. 
    Let $t$ denote the sum of entries in $Z$.
    Then,  
\begin{align*}
t = \sum_w \max (P_x(w), Q_x(w)) &= \sum_w\frac{P_x(w)+ Q_x(w)}2+\frac{|P_x(w)- Q_x(w)|}2\\
&=1+ \dtv(P_x,Q_x)\le1+ \frac{\gamma}{2}\le \frac1{1-\frac{\gamma}{2}},
\end{align*}
where the first inequality comes from~\eqref{equ:tvdistance}.

For $w\in \{0,1\}^{n-1}$, let
\[
P_y(w) =  \frac{2}{\gamma} \cdot \Paren{ \frac {Z_w} t - \Paren{1-\frac{\gamma}{2}}P_x(w)},\ \ \ \ Q_y(w) =  \frac{2}{\gamma} \cdot \Paren{ \frac {Z_w}t - \Paren{1-\frac{\gamma}{2}}Q_x(w)}.
\] 

It follows that 
\[
\left(1-\frac{\gamma}{2}\right)P_x + \frac{\gamma}{2} P_y = \left(1-\frac{\gamma}{2}\right)Q_x + \frac{\gamma}{2} Q_y.
\]

It remains to prove that $P_y$ and $Q_y$ are valid distributions.

Note that $\sum_w P_y(w) = \frac{2}{\gamma} \Paren{1 - \Paren{1-\frac{\gamma}{2}}} = 1$. Since $t \le \frac1{1-\frac{\gamma}{2}}$,
\[
P_y(w) = \frac{2}{\gamma} \cdot \Paren{ \frac{Z_w}t - \Paren{1-\frac{\gamma}{2}}P_x(w)}  \le \frac{2 \Paren{1-\frac{\gamma}{2}}}{\gamma} \cdot \Paren{ Z_w- P_x(w)} \ge 0.
\]
The proof for $Q_y$ is similar.
\end{proof}



%     \gnote{I didn't have time to read the rest of this proof carefully, but it kind of seems like a bunch of random steps without motivation for each. Add more prose to indicate what's going on, how the steps interact with each other etc.}
% First note that
% \begin{align}
% \dtv\Paren{\q_x, \q_y} \le \sqrt{\frac12 \chi^2\Paren{\q_x, \q_y}} \le \sqrt{ \frac{\ns-1}{2} \cdot \frac{2\gamma^2}{4\ns} } \le \frac{\gamma}{2}. 
% \end{align}
%     \gnote{We haven't defined the chi-squared distance before in this paper. Not sure if we have to mention what's going on here. We could just write the inequality explicitly?}

%     We now describe how to construct $P_x$ and $P_y$ over $\{0,1\}^{n-1}$. 
%     Let $A$ be a vector of length $2^{n-1}$ indexed by vectors in $\{0,1\}^{n-1}$, where for $w\in\{0,1\}^{n-1}$, $A_w = \max (\q_x(w), \q_y(w))$. 
%     Let $t$ denote the sum of entries in $A$.
%     Then,  
% \begin{align*}
% t = \sum_w\max (\q_x(w), \q_y(w)) &= \sum_w\frac{\q_x(w)+ \q_y(w)}2+\frac{|\q_x(w)- \q_y(w)|}2\\
% &=1+ \dtv(\q_x,\q_y)\le1+ \frac{\gamma}{2}\le \frac1{1-\frac{\gamma}{2}}.
% \end{align*}
% For $w\in \{0,1\}^{n-1}$
% \[
% P_x(w) =  \frac{2}{\gamma} \cdot \Paren{ \frac {A(w)} t - \Paren{1-\frac{\gamma}{2}}\q_x(w)},\ \ \ \ P_y(w) =  \frac{2}{\gamma} \cdot \Paren{ \frac {A(w)}t - \Paren{1-\frac{\gamma}{2}}\q_y(w)}.
% \] We prove that $P_x$ and $P_y$ are distributions.

% Note that $\sum_w P_x(w) = \frac{2}{\gamma} \Paren{1 - \Paren{1-\frac{\gamma}{2}}} = 1$. Since $t \le \frac1{1-\frac{\gamma}{2}}$,
% \[
% P_x(w) = \frac{2}{\gamma} \cdot \Paren{ \frac{A(w)}t - \Paren{1-\frac{\gamma}{2}}\q_x(w)}  \le \frac{2 \Paren{1-\frac{\gamma}{2}}}{\gamma} \cdot \Paren{ A(w)- \q_x(w)} \ge 0.
% \]
% The proof for $P_y$ is similar.

% There exists a coupling between the degree distributions of a directed ER graph with expected distance $\gamma n$, and by Markov's inequality we obtain a coupling. 

\newhz{
With this lemma in hand, we derive the first term in the max in Theorem~\ref{thm:lower-bound}. Consider the following two processes:

\begin{enumerate}
    \item Given a graph $\derg\sim \derg(n,p)$, the adversary independently selects each node with probability $\frac{\gamma}{2}$. For each selected node, the adversary generates its neighbourhood to be a random subset of size determined by an independent draw from distribution $P_y$.
    \item Given a graph $\derg\sim \derg(n,p+0.1\gamma\sqrt{p/n})$, the adversary randomly picks up each node with probability $\frac{\gamma}{2}$. For each selected node, the adversary generates its neighbourhood to be a random subset of size determined by an independent draw from distribution $Q_y$.
\end{enumerate}

According to Lemma~\ref{lem:same_distribution}, the graphs generated by the two processes share the same underlying distribution. Note that the number of perturbed nodes satisfies $\Bin(n,\gamma/2)$. By Markov's inequality, it will not exceed $5\gamma\ns$ with probability at least $0.8$. Therefore, we have shown a lower bound for robustly estimating directed Erd\H{o}s-R\'enyi graphs. Combined with Lemma~\ref{lem:undirected_to_directed}, we finish the proof of the first term in Theorem~\ref{thm:lower-bound}.
}

To derive the second term in the max in  Theorem~\ref{thm:lower-bound}, one can prove an analogue of Lemma~\ref{lem:same_distribution} with $p = 0$ and $q = 0.1\corr/n$.
The proof is nearly identical, relying on the following total variation bound:
\begin{align*}
d_{\rm TV}\left(\Bin (\newhz{n-1},0),\Bin (\newhz{n-1}, 0.1\gamma/n) \right)
& = 1 - (1-0.1\gamma/n)^{n-1} \le \newhz{1 - (1-0.1\gamma/(n-1))^{n-1}} \le 0.1 \gamma,
\end{align*}
where the last inequality assumes $n \ge 2$.

Finally, we derive the third term in the max in Theorem~\ref{thm:lower-bound}.
We start with the following bound on the KL divergence between binomials:
\begin{align*}
    d_{\rm KL}\left(\Bin (\newhz{n-1}, p+0.1\sqrt{p}/n) || \Bin (\newhz{n-1},p) \right) &= \newhz{(n-1)}\cdot d_{\rm KL}\left(\Ber (p+0.1\sqrt{p}/n) || \Ber(p) \right) \\
    &\le \newhz{(n-1)} \cdot d_{\chi^2}\left(\Ber (p+0.1\sqrt{p}/n) || \Ber(p) \right) \le \frac1{50n},
\end{align*}
where the first inequality follows from the fact that the KL divergence is upper bounded by the chi-square divergence.
This allows us to derive a bound on the KL divergence between directed Erd\H{o}s-R\'enyi graphs:
\begin{align*}
    d_{\rm KL}\Paren{ \newhz{\derg(n, p+0.1\sqrt{p}/n)} || \derg(n,p)} = n \cdot  d_{\rm KL}\left(\Bin (n, p+0.1\sqrt{p}/n) || \Bin (n,p) \right) \le 0.02.
\end{align*}

Pinsker's inequality implies that $d_{\rm TV}\Paren{ \derg(n+0.1\sqrt{p}/n) , \derg(n,p)} \leq \newhz{0.15}$, and standard results imply that no algorithm can distinguish between a sample from these two random graph models with probability greater than $0.6$, completing the proof.

%By Le Cam's method and Lemma~\ref{lem:undirected_to_directed}, we prove a lower of $\Omega\Paren{\sqrt{p}/n}$ for the non-robust case.
% Suppose there is a directed graph such that $A_{i,j}\sim p$.
% We can use the directed graph to simulate an undirected graph by setting $A_{j,i}=A_{i,j}$, or in other words by completely ignoring $A_{j,i}$.
% If we can not learn with the directed graph, then can't learn with the undirected graph as well.



==> median-without-corruptions-old.tex <==

\noindent\textbf{Median estimate.} The median estimate for $p$ is given in~\eqref{eqn:empirical-median-estimator}. We will show that with probability at least $0.99$, the median degree of the graph lies in $(np-C/2, np+C/2)$ for some constant $C$, thus proving that the median estimate is within $\pm C/n$ of $p$. \newer{The main hurdle in showing this is that the node degrees are not independent, which requires a careful analysis to bound the degree variances.} 

\newer{For $i\in[n]$,} let  $ Y_i \coloneqq \id\Paren{\deg(i) \le p(n-1)-180}$ and $ Z_i \coloneqq \id\Paren{\deg(i) \ge p(n-1)+180}$. \newer{Then, $\sum_i Y_i$  is the number of nodes with degree at most  ${p(n-1)-180}$ and $\sum_i Z_i$ is the number of nodes with degree at least ${p(n-1)+180}$. We will show that with probability at least 0.99, $\sum_i Y_i <n/2$, and $\sum_i Z_i < n/2$. This will show that the median degree is in $(np-C/2, np+C/2)$ for $C=360$, proving our result.}

We will show the following bounds for $n>4000$ and then prove concentration.
\begin{align}
&\max\left\{\expectation{\sum_i Y_i}, \expectation{\sum_i Z_i}\right\}\le \frac n2-15\sqrt{n}\label{eqn:mean-bound}\\
&\max\left\{\variance{\sum_i Y_i}, \variance{\sum_i Z_i}\right\}\le n
\label{eqn:variance-bound}
\end{align}
\newer{With these results, we can apply Cantelli's inequality to obtain
\[
\probof{\sum_i Y_i\ge \frac n2}\le \frac{\variance{\sum Y_i}}{\variance{\sum Y_i}+(15\sqrt{n})^2}<0.05.
\]
We similarly obtain that $\probof{\sum_i Z_i\ge \frac n2}\le 0.05$ and by the union bound we get that with probability at least 0.99, both $\sum Y_i$ and $\sum Z_i$ are at most $n/2$, proving the result.}

We now prove~\eqref{eqn:mean-bound} and~\eqref{eqn:variance-bound}. 

To prove~\eqref{eqn:mean-bound}, note that $\deg(i)\sim \Bin(n-1,p)$. Moreover, 
the mean, median and mode of a $Bin(n,p)$ random variable all lie in $[np-1,np+1]$~\cite{KaasB80}. Therefore
$\probof{\deg(i)<(n-1)p+1}\ge 1/2$.
By Chebyshev's inequality, for any $t>0$,
\[
\probof{\deg(i)<(n-1)p-t \sqrt{n}}\le \frac 1{4t^2}.
\]
Combining these two, we obtain $\probof{(n-1)p-t \sqrt{n}<\deg(i)\le (n-1)p+1}\ge 1/2-1/4t^2$.
Since a Binomial random variable has a unique mode between  $[(n-1)p-1,(n-1)p+1]$, 
\begin{align}
{\probof{(n-1)p-180\le\deg(i)\le (n-1)p-1}}&\ge \frac{179}{t\sqrt{n}}\cdot {\probof{(n-1)p-t\sqrt{n}<\deg(i)\le (n-1)p+1}}\notag\\
&\ge \frac{179}{t\sqrt{n}}\cdot\left(\frac 12-\frac 1{4t^2}\right)\notag.
\end{align}
Therefore, 
\begin{align*}
\probof{\deg(i)\le (n-1)p-180}&=  \probof{\deg(i)\le (n-1)p-1}- {\probof{(n-1)p-180<\deg(i)\le (n-1)p-1}}\\
&\le\frac 12- \frac{179}{t\sqrt{n}}\cdot\left(\frac 12-\frac 1{4t^2}\right)\le \frac 12-\frac {15}{\sqrt n},
\end{align*}
for $t=5$. By the linearity of expectations, we get~\eqref{eqn:mean-bound}. 

We now prove~\eqref{eqn:variance-bound}. Since $Y_i$'s are identically distributed,
\begin{align}\label{eqn:var-cov}
\variance{\sum_i Y_i} =n\variance{Y_1}+n(n-1)\covariance(Y_1, Y_2)\le \frac n4+n(n-1)\covariance(Y_1, Y_2).
\end{align}
Let $t=(n-1)p-180$, then  $Y_i= \id\Paren{deg(i) \le t}$. Suppose $Y_{12}$ is the number of edges from node 1 to $[n]\setminus \{2\}$, then $Y_{12}\sim \Bin(n-2, p)$. Elementary computations show that
\[
\covariance(Y_1, Y_2) = p(1-p)\cdot \probof{Y_{12}=t}^2.
\]
From Stirling's approximation at $t=np$, we have $\probof{Y_{12}=t}\le 1/\sqrt{\pi p(1-p)(n-2)}$, and therefore, 
\[
\covariance(Y_1, Y_2) = p(1-p)\cdot \probof{Y_{12}=t}^2\le \frac1{\pi(n-2)}\le \frac 1{3n}
\]
for $n>4000$. Plugging this in~\eqref{eqn:var-cov} proves~\eqref{eqn:variance-bound}.


% The first lemma provides an upper bound for the maximum of the PMF of a binomial distribution,
% \begin{lemma}
% \label{lem:binom_max}
% Let $X \sim \Bin(n,p)$. If $np(1-p) \ge 1000$, 
% $
% \max_{k\in[n]} \probof{X = k} \le \frac{1}{\sqrt{\pi p(1-p)n}}.
% $
% \end{lemma}
% \begin{proof}
% \[
% \probof{X = k} = \binom{n}{k} p^{k} \cdot (1-p)^{n-k} = \frac{n!}{k!(n-k)!}p^{k} \cdot (1-p)^{n-k}.
% \]
% Let $k^* = \arg \max_{k\in[n]} \probof{X = k}$, we note that $k^* \in \{\lfloor np \rfloor, \lceil np \rceil \}$. For $k \in \{\lfloor np \rfloor, \lceil np \rceil \} $, by Stirling's approximation,
% \begin{align*}
%     \probof{X = k} \le \frac{\sqrt{n}}{\sqrt{2\pi k (n-k)}} \cdot \frac{n^n}{\Paren{\frac{k}{p}}^k \Paren{\frac{n-k}{1-p}}^{n-k}}.
% \end{align*}
% Consider the following function $f(x) = \Paren{\frac{x}{p}}^x \Paren{\frac{n-x}{1-p}}^{n-x}$, where $x \in [\lfloor np \rfloor, \lceil np \rceil ]$. Let
% \begin{align*}
%     F(x) \coloneqq  log(f(x)) = x \log \frac{x}{p}+ (n-x)\log \frac{n-x}{1-p},
% \end{align*}
% with
% \begin{align*}
%     F^\prime (x) = \log \frac{x}{p}-\log \frac{n-x}{1-p}.
% \end{align*}

% Note that $F^\prime (x)$ takes 0 when $x = np$. Besides, $F^\prime (x) \le 0$ when $x \le np$; $F^\prime (x) \ge 0$ when $x \ge np$.  Therefore, $f(x) \ge f(np) =n^n$.

% Let $k \in \{\lfloor np \rfloor, \lceil np \rceil \} $,
% \begin{align*}
%     \probof{X = k} \le \frac{\sqrt{n}}{\sqrt{2\pi k (n-k)}}
%     \le \frac{\sqrt{n}}{\sqrt{2\pi (np-1) (n-np-1)}} \le \frac{1}{\sqrt{\pi p(1-p)n}},
% \end{align*}
% where the last inequality comes from $np(1-p)\ge 1000$.
% \end{proof}

% In the next lemma, we bound the mass of a binomial distribution that has a large deviation from the mean.
% \begin{lemma}
% \label{lem:binom_concen}
% Let $X \sim \Bin(n-1,p)$. When $n\ge 4000$,
% \[
% \probof{\frac{X}{n-1} \le p -\frac{180}{n-1}} < \frac12 - \frac{15}{\sqrt{n}}.
% \]
% \end{lemma}

% \begin{proof}[Proof of Lemma~\ref{lem:binom_concen}]

% Without loss of generality, we assume $p> \frac{180}{n-1}$. Else the lemma is simply true.

% Note that $\expectation{\frac{X}{n-1}} = p$, and $\Var(\frac{X}{n-1}) < {\frac{p(1-p)}{n-1}}$. By Bernstein's inequality (Lemma~\ref{lem:chernoff}), 
% \begin{align}
% \label{equ:chebyshev_median}
% \probof{{X} \le (n-1)p -  \max\Paren{3\sqrt{(n-1)p (1-p)}, 9}} \le \frac1{9}.
% \end{align}

% % Since $(n-1)p \ge 180$, we have $3\sqrt{(n-1)p}>9$. Therefore,
% % \begin{align}
% % \label{equ:chebyshev_median}
% % \probof{{X} \le (n-1)p -  3\sqrt{(n-1)p}} \le \frac1{9}.
% % \end{align}

% We first consider the case when $3\sqrt{(n-1)p(1-p)}\le 180$, where $(n-1)p(1-p)\le 3600$. By~\eqref{equ:chebyshev_median},
% \[
% \probof{\frac{X}{n-1} \le p -\frac{180}{n-1}} \le \probof{\frac{X}{n-1} \le p -\max\Paren{ 3\sqrt{\frac{p(1-p)}{n-1} }, 9}} \le \frac1{2}-\frac{15}{\sqrt{n}}.
% \]

% Then we consider the case when $3\sqrt{(n-1)p(1-p)}> 180$, where $\frac{180}{n-1} < 3\sqrt{\frac{p(1-p)}{n-1}}.$
% According to Lemma~\ref{lem:binom_max}, and the property that the median of $\Bin(n-1,p)$ lies in $[\lfloor(n-1)p\rfloor, \lceil(n-1)p\rceil]$,
% \begin{align*}
%     &\probof{X < \lfloor(n-1)p\rfloor}<0.5,\\
%     &\probof{X < \lfloor(n-1)p\rfloor} \ge 0.5 - \frac{2}{\sqrt{\pi p(1-p)(n-1)}}>0.46.
% \end{align*}

% Combined with~\eqref{equ:chebyshev_median},

% \begin{align*}
% \probof{ (n-1)p - 3\sqrt{p(1-p)(n-1)} < X < \lfloor(n-1)p\rfloor } \ge 0.46- \frac1{9} > \frac1{3}.
% \end{align*}

% Note that $0< p -3\sqrt{\frac{p(1-p)}{n-1}}< p -\frac{180}{n-1}$,

% \[
% \probof{p-\frac{180}{n-1} < \frac{X}{n-1} < \frac{\lfloor(n-1)p\rfloor}{n-1} }> \frac1{3}\cdot \frac{180}{n-1}\cdot \frac{1}{3\sqrt{\frac{p(1-p)}{n-1}}}  > \frac{20}{\sqrt{n-1}}.
% \]

% Note that $\probof{X < \lfloor(n-1)p\rfloor}<0.5$, we have
% \[
% \probof{\frac{X}{n-1} \le p -\frac{180}{n-1}} < \frac12 - \frac{15}{\sqrt{n}}.
% \]
% \end{proof}

% \newhz{
% \begin{lemma}
% \label{lem:cov}
% Let $ Y_i \coloneqq \id\Paren{deg(i) \le \text{med}(X)-180}$. For any $i,j \in [\ns]$,
% \[
% \covariance\Paren{Y_i, Y_j} \le \frac1{n-2}.
% \]
% \end{lemma}
% \begin{proof}
% Let $t = \text{med}(X)-180$,
% \begin{align*}
% &~~~~\covariance\Paren{Y_i, Y_j} \\
% &= \expectation{Y_i \cdot Y_j} - \expectation{Y_i} \cdot \expectation{Y_j}  = \probof {Y_i =1, Y_j =1} - \Paren{\probof {Y_i=1}}^2\\
% & = \sum_{u \in \{0,1\}}\probof{e(i,j)=u} \cdot \probof {Y_i =1, Y_j =1 |e(i,j)=u } - \Paren{\probof {Y_i=1}}^2\\
% & = p\cdot \Paren{\probof{\Bin(n-2,p)\le t-1}}^2+(1-p)\cdot \Paren{\probof{\Bin(n-2,p)\le t}}^2-\Paren{\probof{\Bin(n-1,p)\le t}}^2.
% \end{align*}
% Let $a\coloneqq \probof{\Bin(n-2,p)\le t-1}$, and $b \coloneqq \probof{\Bin(n-2,p)\le t}$, then
% \begin{align*}
% \covariance\Paren{Y_i, Y_j} &= pa^2+ (1-p)b^2 - \Paren{pa+(1-p)b}^2\\
% & = pa^2+ (1-p)b^2 - p^2a^2+ (1-p)^2b^2 - 2p(1-p)ab\\
% & = p(1-p)(a-b)^2.
% \end{align*}
% Note that $b-a = \probof{\Bin(n-2,p)= t} \le \frac{1}{\sqrt{n-2}}$, we conclude the proof.
% \end{proof}

% Let $Y = \sum_{i=1}^\ns Y_i \coloneqq  \sum_{i=1}^\ns \id\Paren{deg(i) \le \text{med}(X)-180}$ denote the number of the nodes whose degrees are small. In order to apply Chebyshev's inequality to bound its value, we need to analyze its mean and variance. First,
% \begin{align}
% \expectation{Y}&= \sum_{i=1}^{\ns}\probof{deg(i) \le \text{med}(X)-180 } \le \frac{1}{2}\ns - 14\sqrt{n}. \nonumber
% \end{align}

% Next we bound the variance of $Y$.
% \begin{align}
% \variance{Y} = \variance{\sum_{i=1}^{\ns}Y_i} &= \sum_{i=1}^{\ns} \variance{Y_i} + \sum_{i\neq j} \covariance\Paren{Y_i, Y_j} \nonumber\\
% &\le \frac{\ns}{4}+\frac{n(n-1)}{n-2} \le 1.5\ns. \nonumber
% \end{align}
% Finally, by Chebyshev's inequality, there are less than $\frac{n}{2}$ nodes whose degrees are smaller than $\text{med}(X)-180$, with probability at least 0.9. Similarly, we can show that there are less than $\frac{n}{2}$ nodes whose degrees are more than $\text{med}(X)-180$, with probability at least 0.9. We conclude the proof by union bound, and the fact that $p(n-1)-1 \le \text{med}(X) \le p(n-1)+1$
% }
% In the next lemma, we bound the correlation between each node.
% \begin{lemma}
% \label{lem:cov}
% Let $ Y_i \coloneqq \id\Paren{deg(i) \le p(n-1)-180}$. For any $i,j \in [\ns]$,
% \[
% \covariance\Paren{Y_i, Y_j} \le \frac1{n-1}.
% \]
% \end{lemma}
% \begin{proof}
% Let $t = p(n-1)-180$,
% \begin{align*}
% &~~~~\covariance\Paren{Y_i, Y_j} \\
% %&= \expectation{Y_i \cdot Y_j} - \expectation{Y_i} \cdot \expectation{Y_j}  
% &= \probof {Y_i =1, Y_j =1} - \Paren{\probof {Y_i=1}}^2\\
% & = \sum_{u \in \{0,1\}}\probof{e(i,j)=u} \cdot \probof {Y_i =1, Y_j =1 |e(i,j)=u } - \Paren{\probof {Y_i=1}}^2\\
% & = p\cdot \Paren{\probof{\Bin(n-2,p)\le t-1}}^2+(1-p)\cdot \Paren{\probof{\Bin(n-2,p)\le t}}^2-\Paren{\probof{\Bin(n-1,p)\le t}}^2.
% \end{align*}

% Let $a\coloneqq \probof{\Bin(n-2,p)\le t-1}$, and $b \coloneqq \probof{\Bin(n-2,p)\le t}$, then
% \begin{align*}
% \covariance\Paren{Y_i, Y_j} &= pa^2+ (1-p)b^2 - \Paren{pa+(1-p)b}^2\\
% & = pa^2+ (1-p)b^2 - p^2a^2- (1-p)^2b^2 - 2p(1-p)ab\\
% & = p(1-p)(a-b)^2.
% \end{align*}

% Now we bound $b-a = \probof{\Bin(n-2,p)= t}$. Without loss of generality, we assume $p(n-1) \ge 180$. Else $a-b=0$.

% When $(n-2)p(1-p) \ge 1000$, by Lemma~\ref{lem:binom_max}, we have 
% $b-a \le \frac{1}{\sqrt{\pi p(1-p)(n-2)}}$. Therefore, 
% \[
% \covariance\Paren{Y_i, Y_j} = p(1-p)(b-a)^2 \le \frac1{n}.
% \]
% Finally, we consider $(n-2)p(1-p)<1000$, by Lemma~\ref{lem:chernoff},
% $b-a = \probof{\Bin(n-2,p)= t} \le \frac1{100}$.Therefore,
% \[
% \covariance\Paren{Y_i, Y_j} = p(1-p)(b-a)^2 \le \frac1{n}.
% \]

% \end{proof}

% Let $Y = \sum_{i=1}^\ns Y_i \coloneqq  \sum_{i=1}^\ns \id\Paren{deg(i) \le p(n-1)-180}$ denote the number of the nodes whose degrees are small. In order to apply Chebyshev's inequality to bound its value, we need to analyze its mean and variance. First,
% \begin{align}
% \expectation{Y}&= \sum_{i=1}^{\ns}\probof{deg(i) \le p(n-1)-180 } \le \frac{1}{2}\ns - 15\sqrt{n}. \nonumber
% \end{align}

% Next we bound the variance of $Y$.
% \begin{align}
% \variance{Y} = \variance{\sum_{i=1}^{\ns}Y_i} &= \sum_{i=1}^{\ns} \variance{Y_i} + \sum_{i\neq j} \covariance\Paren{Y_i, Y_j} \nonumber\\
% &\le \frac{\ns}{4}+\frac{n(n-1)}{n-1} \le 1.5\ns. \nonumber
% \end{align}
% Finally, by Chebyshev's inequality, there are less than $\frac{n}{2}$ nodes whose degrees are smaller than $p(n-1)-180$, with probability at least 0.9. Similarly, we can show that there are less than $\frac{n}{2}$ nodes whose degrees are more than $p(n-1)-180$, with probability at least 0.9. We conclude the proof by union bound.



==> old-upper-bound.tex <==
\section{Estimation via a spectral algorithm}
\input{old-upper-bound.tex}
Let $\tilde A\sim G(n,p) $ be the adjacency matrix of a (random?) Erd\"os-R\'enyi graph.
The adversary observes $\tilde A$, it can then choose a set $B\subseteq[n]$ of nodes of size  $|B|\le \gamma n$.
We refer to nodes in $B$ as \emph{adversarial nodes}
and the remaining nodes $\goodnodes  := [n]\setminus B$ as \emph{good nodes}.
The adversary can add an edge or remove an existing edge between a pair of nodes if at least one of them is an adversarial node. 
Let $A$ be the adjacency matrix of the modified graph.
Observe that $A$ is a symmetric binary matrix and $A_{\goodnodes \times \goodnodes } = \tilde A_{\goodnodes \times \goodnodes }$, and the remaining entries of $A$ can be arbitrary.


We do not know the identity of the good or the adversarial nodes. The goal is to use the matrix $A$ to learn the parameter $p$ of the Erd\"os-R\'enyi graph $\tilde A$.
We assume $0\le \gamma \le c$, where $c<1/2$ is some absolute constant.


\textbf{Remark:} We have assumed the undirected graph model, hence $A$ is a symmetric matrix. 
For the directed graph model one can consider $(A+A^\intercal)/2$ instead of $A$, which will be symmetric. The new $(A+A^\intercal)/2$ will not be a binary matrix anymore, but our analysis do not use the fact and will still be applicable.

% \subsection{Concentration properties of the Erd\"os-R\'enyi graph}







% For a subset $S\subseteq[n]$, let $p_S := \frac{1}{|S|^2}\sum_{i,j\in S}A_{i,j} $.
% The following equation is a simple consequence of the second property in the above corollary. If the above corollary holds then for any $\alpha\in[\frac{1}{\sqrt n},\frac{1}{2}]$ and $\goodnodesub\subseteq \goodnodes $ such that $n-|\goodnodesub|\le \alpha n$, 
% \begin{equation}\label{eq:useful}
% \Bigg|{\sum_{i,j\in \goodnodesub}(A_{i,j}-p)}\Bigg|\le  c_1\alpha n^2\cdot\kappa(\alpha,p,n),
% \end{equation}
% and

% \hztodo{do we want to replace the second property in Corollary~\ref{cor:goodspecnorm} by Equation~\eqref{eq:usefula}? }
% The reminder of the section we condition on the event in the above corollary holds.
% \begin{algorithm}[H]
%   \begin{algorithmic}
%     \Require{$\gamma\le 1/60$, $n$, \newhz{perturbed graph} $A$}
%     \State{$S\gets [n]$, list$\gets\{\}$, and $Del = 0$}
%     \State{list.insert$(S)$} \textit{\ \ \ \ \ \ \ \ \ \ \ List of all subsets $S$ along the path}
%     \While{$Del < 9\gamma n$}
%         \State{Find the top eigenvalue $v$ of unit length of the matrix $(A - p_S)_{S\times S}$}
%         \State{$i^{D}\gets$ Randomly pick an element $i\in S$ where the probability of picking $i$ is $v_i^2$}
%         \State{$Del\gets Del+1 $ and $S\gets S\setminus\{i^{D}\}$}
%         \State{list.insert$(S)$}
%     \EndWhile
%     \State{$S^*\gets \arg\min_{S\in \text{list}} \|(A - p_S)_{S\times S}\|$}\\
%      \Return $S^*$ 
%   \end{algorithmic}
%   \caption{\label{algo:part}Spectral Algorithm}
% \end{algorithm}




\subsection{Final trimming}

Recall that Algorithm~\ref{algo:part} returns a subset $S^*$ of size $\ge (1-9\gamma)n$ and from Theorem~\ref{thm:specnorm} w.h.p. $\|(A_{S^*\times S^*} - p_S^*)\|\le 10 c_2n \cdot \kappa(10\gamma,p,n) $. Also note that for $\gamma\le 1/60$, $|S^*\cap \goodnodes |\ge |S^*|-|B|\ge (1-10\gamma)n\ge 5n/6 $.

The following lemma shows that $p_S^*$ is a good estimate of $p$.
Later in this section use it to obtain an even better estimate.
% \begin{lemma}\label{lem:trimnod}
% For any matrix $A\in \mathbb R^{n\times n}$, $\gamma\in [\frac{1}{\sqrt{n}}, \frac{1}{60}]$. Given the events in corollary holds and Algorithm~\ref{algo:part} returns a subset $S^*$ such that $\|(A_{S^*\times S^*} - p_S^*)\|\le 10 c_2n \cdot \kappa(10\gamma,p,n)$ then
% $|p_{S^*}-p|\le (20c_2+2c)\cdot \kappa(10\gamma,p,n)$.
% \end{lemma}
% \begin{proof}
% \begin{align*}
%  \|(A-p_{S^*})_{({S^*}\cap \goodnodes )\times({S^*}\cap \goodnodes )}\| &= \|(A-p+p-p_{S^*})_{({S^*}\cap \goodnodes )\times({S^*}\cap \goodnodes )}\|\\
%  &\ge  |p-p_{S^*}|\cdot|{S^*}\cap \goodnodes |- \|(A-p)_{({S^*}\cap \goodnodes )\times({S^*}\cap \goodnodes )}\|\\
%   &\ge  |p-p_{S^*}|\cdot|{S^*}\cap \goodnodes |- \|(A-p)_{ \goodnodes \times \goodnodes }\|.
%  \end{align*}
%  Therefore, \newhz{according to the first property of Corollary~\ref{cor:goodspecnorm},}
% \begin{align*}
%  |p-p_{S^*}|\cdot|{S^*}\cap \goodnodes |
%  &\le 10c_2n\cdot \kappa(10\gamma,p,n)+ cn\cdot \kappa(10\gamma,p,n).
% \end{align*}
% Using $|S^*\cap \goodnodes |> n/2$ in the above equation proves the lemma.
% \end{proof}



%Next we describe the trimming operation:
%Start with $S=S^*$.
%Until there is a node $i\in S$ such that $|p_{S^*}-p^{S}_i|\gg \sqrt{\frac{\log(1/\gamma)}{n}}$,
%remove $i$ from $S$.


The next corollary follows from the above two lemmas.
\begin{corollary}\label{cor:devbound}
For any matrix $A\in \mathbb R^{n\times n}$, $\gamma\in [\frac{1}{\sqrt{n}}, \frac{1}{60}]$. Given the events in corollary holds and Algorithm~\ref{algo:part} returns a subset $S^*$ such that $\|(A_{S^*\times S^*} - p_S^*)\|\le 10c_2n\cdot \kappa(10\gamma,p,n) $.
Then for any $\goodnodesub,\goodnodesubanother\subseteq \goodnodes $ such that $\goodnodesub\le \gamma n$ and $\min\{\goodnodesubanother,n-\goodnodesubanother\}\le 12\gamma n$ and some universal constant $c_3>0$,  
\[
\Bigg|\sum_{i\in \goodnodesub,\, j\in \goodnodesubanother}(A_{i,j}-p_{S^*})\Bigg| \le c_3\gamma n^2
\cdot \kappa(10\gamma,p,n).
\]
\end{corollary}
\begin{proof}
From Corollary~\ref{cor:goodspecnorm},
\[
\Bigg|{\sum_{i\in \goodnodesub,\,j\in \goodnodesubanother}(A_{i,j}-p)}\Bigg|\le  c_1 (12\gamma n^2)
\cdot \kappa(12\gamma,p,n)\le  12c_1 \gamma n^2
\cdot \kappa(10\gamma,p,n),
\]
here the last inequality uses the fact that $\kappa(\alpha,p,n)$ is a decreasing function of $\alpha$.
Then
\begin{align*}
\Bigg|\sum_{i\in \goodnodesub,\, j\in \goodnodesubanother}(A_{i,j}-p_{S^*})\Bigg| &\le \Bigg|\sum_{i\in \goodnodesub,\, j\in \goodnodesubanother}(A_{i,j}-p+p-p_{S^*})\Bigg|\\
&\le \Bigg|\sum_{i\in \goodnodesub,\, j\in \goodnodesubanother}(A_{i,j}-p)\Bigg|+|\goodnodesub|\cdot|\goodnodesubanother|\cdot|p-p_{S^*}|\\
&\le 12c_1 \gamma n^2
\cdot \kappa(10\gamma,p,n)+(\gamma n)n\cdot|p-p_{S^*}|\\ 
&\le 12c_1 \gamma n^2
\cdot \kappa(10\gamma,p,n)+(\gamma n)n\cdot (20c_2+2c)\cdot \kappa(10\gamma,p,n)\\ 
&\le c_3\gamma n^2\cdot \kappa(10\gamma,p,n),
\end{align*}
here the second last step follows from Theorem~\ref{lem:trimnod}.
\end{proof}


Consider any $\goodnodesub\subseteq {S^*}\cap \goodnodes $ such that $|\goodnodesub|= \gamma n$. Since $|{S^*}\cap B|\le|B|\le\gamma n$, then from Lemma~\ref{lem:somecor}
\begin{align*}
\Bigg|\sum_{i\in \goodnodesub,\, j\in {S^*}\cap B}(A_{i,j}-p_{S^*})\Bigg|\le  30c_2\gamma n^2\cdot \kappa(10\gamma,p,n).
\end{align*}

Combining the above equation and Corollary~\ref{cor:devbound}, for any $\goodnodesub\subseteq {S^*}\cap \goodnodes $ such that $|\goodnodesub|= \gamma n$ we get
\begin{align*}
\Bigg|\sum_{i\in \goodnodesub,\, j\in {S^*}}(A_{i,j}-p_{S^*})\Bigg|&\le \Bigg|\sum_{i\in \goodnodesub,\, j\in {S^*}\cap \goodnodes }(A_{i,j}-p_{S^*})\Bigg|+\Bigg|\sum_{i\in \goodnodesub,\, j\in {S^*}\cap B}(A_{i,j}-p_{S^*})\Bigg|\\
&\le    c_3\gamma n^2\cdot \kappa(10\gamma,p,n)+30c_2\gamma n^2\cdot \kappa(10\gamma,p,n)\\
&\le    (c_3+30c_2)\gamma n^2\cdot \kappa(10\gamma,p,n).
\end{align*}

Then, for any $\goodnodesub\subseteq {S^*}\cap \goodnodes $ such that $|\goodnodesub|= \gamma n$,
\begin{align}\label{eq:cont}
\frac{1}{|\goodnodesub|}\Bigg|\sum_{i\in \goodnodesub}(p^{S^*}_{i}-p_{S^*})\Bigg|
&=\frac{1}{|\goodnodesub|\cdot|{S^*}|}\Bigg|\sum_{i\in \goodnodesub,\, j\in {S^*}}(A_{i,j}-p_{S^*})\Bigg|\nonumber\\
&\le\frac{2}{\gamma n^2}\Bigg|\sum_{i\in \goodnodesub,\, j\in {S^*}}(A_{i,j}-p_{S^*})\Bigg|\nonumber\\
&\le (2c_3+60c_2)\cdot \kappa(10\gamma,p,n),
\end{align}
here in the first inequality we used $|{S^*}| \ge (1-9\gamma)|\goodnodes |> n/2$ and $|\goodnodesub|=\gamma n$.


\begin{proof}
We prove by contradiction. Suppose even after $3\gamma n$ good nodes are deleted there is a node $i\in S^f$ such that
\[
|p_{S^*}-p^{S^*}_i|> (2c_3+60c_2)\cdot \kappa(10\gamma,p,n)\Big\}.
\]
This means there were at least $3\gamma n$ such nodes in $S^*$ initially.
Since there are at most $\gamma n$ nodes in $S^*\cap B$ therefore at least $2\gamma n$ of these nodes must be in $S^*\cap \goodnodes $.
Let 
\[
D^+ := \Big\{i\in S^*\cap \goodnodes : p_{S^*}-p^{S^*}_i> (2c_3+60c_2)\cdot \kappa(10\gamma,p,n)  \Big\},
\]
and similarly let
\[
D^- := \Big\{i\in S^*\cap \goodnodes : p^{S^*}_i-p_{S^*}> (2c_3+60c_2)\cdot \kappa(10\gamma,p,n)\Big\}.
\]
Since $D^+\cup D^- \ge 2\gamma n$ at least one of $D^+$ and $D^-$ has $\ge \gamma n$ nodes. Any of which these two cases will contradict Equation~\eqref{eq:cont}.
\end{proof}

Note that $|S^f|\ge |{S^*}|-3\gamma n\ge (1-9\gamma )n-3\gamma n=(1-12\gamma)n\ge n/2$. Also, $|S^f\cap \goodnodes |\ge |{S^f}|-|B|\ge (1-12\gamma)n-\gamma n = (1-13\gamma)n> n/2$.



\begin{theorem}
For any matrix $A\in \mathbb R^{n\times n}$, $\gamma\in [\frac{1}{\sqrt{n}}, \frac{1}{60}]$. Given the events in corollary holds and Algorithm~\ref{algo:part} returns a subset $S^*$ such that $\|(A_{S^*\times S^*} - p_S^*)\|\le 10c_2n\cdot \kappa(10\gamma,p,n) $.
Then for some universal constant $c_4>0$, 
\[
\big|{p_{S^f}}-p\big|\le   c_4\gamma\cdot \kappa(10\gamma,p,n)\le c_4\gamma \max\Bigg(\sqrt{\frac{p}{n}\ln\frac{1}{\gamma}+\frac{\ln n}{n^2}} ,\frac{1}{n}\ln\frac{1}{\gamma}\Bigg).
\]
\end{theorem}
\begin{proof}
\begin{align*}
\big|{p_{S^f}}-p\big|&=\Bigg|\frac{\sum_{i,j\in S^f}A_{i,j}}{|S^f|^2}-p\Bigg|\\
&\le
\Bigg|\frac{\sum_{i,j\in S^f\cap \goodnodes }(A_{i,j}-p)}{|S^f|^2}
+2\frac{\sum_{i\in S^f  \,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}
-\frac{\sum_{i,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|\\
&\le
\Bigg|\frac{\sum_{i,j\in S^f\cap \goodnodes }(A_{i,j}-p)}{|S^f|^2}\Bigg|
+2\Bigg|\frac{\sum_{i\in S^f  \,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|
+\Bigg|\frac{\sum_{i,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|\\
&\le
\Bigg|\frac{\sum_{i,j\in S^f\cap \goodnodes }(A_{i,j}-p)}{|S^f\cap \goodnodes |^2}\Bigg|
+2\Bigg|\frac{\sum_{i\in S^*  \,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|
+2\Bigg|\frac{\sum_{i\in S^*\setminus S^f  \,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|\\
&
+\Bigg|\frac{\sum_{i,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|.
\end{align*}
To prove the theorem we show that each term on the right is upper bounded by $\mathcal O(\gamma\cdot \kappa(10\gamma,p,n))$.

We start by bounding the first term. As $|S^f\cap \goodnodes |\ge  (1-13\gamma)n\ge n/2$, from Equation~\eqref{eq:usefula},
\[
 \Bigg|\frac{\sum_{i,j\in S^f\cap \goodnodes }(A_{i,j}-p)}{|S^f\cap \goodnodes |^2}\Bigg| = |p_{S^f\cap \goodnodes }-p|\le 4c_1 (13\gamma)\cdot \kappa(13\gamma,p,n)\le 52c_1 \gamma\cdot \kappa(10\gamma,p,n),
\]
here the last inequality uses the fact that $\kappa(\alpha,p,n)$ is a decreasing function of $\alpha$.

Next we bound the second term:
\begin{align*}
&\Bigg|\frac{\sum_{i\in S^*  \,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|\\
&\le  \sum_{j\in S^f\cap B}\Bigg|\frac{\sum_{i\in S^*}(A_{i,j}-p)}{n^2/4}\Bigg| \\
&\le \sum_{j\in S^f\cap B}\frac{4|S^*|}{n^2}\Bigg|\frac{\sum_{i\in S^*}(A_{i,j}-p)}{S^*}\Bigg|\\
&\le \sum_{j\in S^f\cap B}\frac{4}{n}|p_j^{S^*}-p|\\
&\le \sum_{j\in S^f\cap B}\frac{4}{n}\big(|p_j^{S^*}-p_{S^*}|+|p-p_{S^*}|)\\
&\overset{(a)}\le \sum_{j\in S^f\cap B}\frac{4}{n}\Big((2c_3+60c_2)\cdot \kappa(10\gamma,p,n) +(20c_2+2c)\cdot \kappa(10\gamma,p,n)\Big)\\
&\le |S^f\cap B|\frac{4}{n}(2c_3+80c_2+2c)\cdot \kappa(10\gamma,p,n)\\
&\le \gamma n\frac{4}{n}(2c_3+80c_2+2c)\cdot \kappa(10\gamma,p,n)\le (8c_3+320c_2+8c)\gamma\cdot \kappa(10\gamma,p,n),
\end{align*}
here (a) uses Lemma~\ref{lem:trimnodes} and Lemma~\ref{lem:trimnod}.

Next, we bound the third term:
\begin{align*}
&\Bigg|\frac{\sum_{i\in S^*\setminus S^f ,  \,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg| \\   
&\le 
\Bigg|\frac{\sum_{i\in S^*\setminus S^f ,  \,j\in S^f\cap B}(A_{i,j}-p)}{n^2/4}\Bigg|  \\
&\le 
\Bigg|\frac{\sum_{i\in S^*\setminus S^f   \,j\in S^f\cap B}(A_{i,j}-p_{S^*})}{n^2/4}\Bigg|+ \frac{|p_{S^*}-p|\cdot|S^*\setminus S^f |\cdot|S^f\cap B|}{n^2/4}   \\
&\overset{(a)}\le 
\Bigg|\frac{\sum_{i\in S^*\setminus S^f   \,j\in S^f\cap B}(A_{i,j}-p_{S^*})}{n^2/4}\Bigg|+ \big((20c_2+2c)\cdot \kappa(10\gamma,p,n)\big)\frac{|S^*|\cdot| B|}{n^2/4}   \\
&\overset{(b)}\le 
\max_{S_1,S_2\subseteq S^*: |S_1|\le \gamma n,\, |S_2|\le 3\gamma n}\Bigg|\frac{\sum_{i\in S_1, \,j\in S_2}(A_{i,j}-p_{S^*})}{n^2/4}\Bigg|+  \big((20c_2+2c)\cdot \kappa(10\gamma,p,n)\big)\frac{n(\gamma n)}{n^2/4}    \\
&\overset{(c)}\le 4\frac{30c_2\gamma n^2
\cdot \kappa(10\gamma,p,n)}{n^2}+(80c_2+8c)\gamma \cdot \kappa(10\gamma,p,n)=(200c_2+8c)\gamma \cdot \kappa(10\gamma,p,n),
\end{align*}
here (a) uses Lemma~\ref{lem:trimnod}, inequality (b) follows since $|S^*\setminus S^f|\le 3\gamma n$, $S^f\subseteq S^*$ and $|B|\le\gamma n$,
and the last inequality uses Lemma~\ref{lem:somecor}.

Finally the last term can be bounded similar to the third term to complete the proof.
\end{proof}




==> rough.tex <==
%Non-trivial robust estimation is only possible because even after edges connected to a few nodes in an Erd\H{o}s-R\'enyi graph is changed arbitrarily, the subgraph between the remaining nodes is unaffected and retains certain structure.
%In this section, we formalize this structure and show that with high probability the subgraph between the uncorrupted set of nodes of a randomly generated Erd\H{o}s-R\'enyi graph has this structure.
%In the following subsections we present algorithm(s) for robust estimation for any graph that possesses such a structure.

As our main focus in this work is the random graphs generated by Erd\H{o}s-R\'enyi model over the vertex set $[n]$, we assume that the adjacency matrix $\AdjM$ is an $n\times n$ matrix with $\AdjM_{i,i}=0$. However, the techniques and the results easily translate for directed graphs and graphs with self loops.
%We often refer the adjacency matrix $\AdjM$ of a graph as a graph.
%For any $S\subseteq[n]$, the sub-graph formed by the nodes in $S$ and the edges that have both ends in $S$. 

\tcr{move to notation?}
Let $J$ denote the $n\times n$ matrix with $0$ on the diagonal and $1$ in all other entries.
For any two real matrices $M$ and $M'$ of the same dimensions, let $\langle M, M'\rangle:=\sum_{i,j} M_{i,j} M'_{i,j}$ denote the element-wise inner product between them.
Note that for any $M\in \mathbb R^{n\times n}$,  we have $\sum_{i\in S, j\in S',i\neq j} M_{i,j} = \langle M, J_{S\times S'}\rangle$ and $M-x J$ is matrix obtained by subtracting $x$ from all entries of $M$ except the diagonal entries.

For an adjacency matrix $\AdjM$ and $S \subseteq [n]$, let $p_S^{\AdjM}:= \frac{\sum_{i,j \in S} \AdjM_{i,j}}{|S|(|S|-1)}=\frac{\langle\AdjM , J_{S\times S}\rangle}{|S|(|S|-1)}$ to denote the empirical fraction of edges present in the subgraph induced by $S$.


For $x\in [0,1/2)$, let $\CX{x}:= [0, \lfloor xn\rfloor ]\cup[\lfloor (1-x)n \rfloor,n]$ and for $x\ge 1/2$ let $\CX{x}:= [0, n]$.

\begin{definition}
%{$(\regpar,\Bounda,\Boundb)$ regular subgraph}: 
For a graph adjacency matrix $A$, $\regpar\in[1/n,1/2]$, and $\Bounda>0$, subgraph over a subset $\goodnodes\subseteq [n]$ is a \emph{$(\regpar,\Bounda,\Boundb)$ regular subgraph} if
\begin{enumerate}
\item \label{pt:zero-pointa} $|\goodnodes^c|\le \regpar n$.
    \item \label{pt:first-pointa}
    $\|(\AdjM - p_{\goodnodes}^{\AdjM}\cdot J)_{\goodnodes\times \goodnodes} \| \le  n\Bounda.$
   \item   \label{pt:second-pointa} For all $\goodnodesub , \goodnodesubanother\subseteq \goodnodes $ such that $|\goodnodesub |,|\goodnodesubanother|\in \CX{13\regpar}$, then
$
\Big|\langle(\AdjM-p_{\goodnodes}^{\AdjM} \cdot J)  , J_{\goodnodesub\times\goodnodesubanother}\rangle\Big|\le  \alpha n^2\Boundb. 
$
\end{enumerate}
\end{definition}

Item~\ref{pt:zero-pointa} implies that the number of nodes outside the regular subgraph are at most $\regpar n$.

Item~\ref{pt:first-pointa} implies that upon subtracting the average degree of subgraph $\goodnodes\times \goodnodes$ from each entry (except diagonal) of the adjacency matrix $\AdjM$, the spectral norm of the matrix corresponding to the subgraph $\goodnodes\times \goodnodes$ is bounded. 

Item~\ref{pt:second-pointa} implies that upon subtracting the average degree of subgraph $\goodnodes\times \goodnodes$ from each entry (except diagonal) of the adjacency matrix $\AdjM$, the sum of the entries over any of its submatrices $\goodnodesub\times\goodnodesubanother\subseteq\goodnodes\times \goodnodes$ has a small absolute value,  as long as each of $\goodnodesub$ and $\goodnodesubanother$ either leave out or include at most $13\regpar n$ nodes.

Note that whether a subgraph is $(\regpar,\Bounda)$ regular or not is determined only by its internal edges, hence this property is unaffected by the corruption caused due to nodes outside this subgraph. 



\begin{theorem}\label{th:erdrenyreg}
Let $\tilde A$ be the adjacency matrix of a sample from $G(n,p)$. 
With probability at least $1-4n^{-2} $, simultaneously for all $\regpar\in[1/n,1/2)$ and all subsets $S\subseteq[n]$ of size $|S|\ge (1-\regpar)n$, 
\begin{enumerate}
    \item Subgraph over $S$ is $(\regpar,\Bounda,\Boundb)$ regular for $\Bounda = c_1\sqrt{\frac{p(1-p)}{n}+\frac{\ln n}{n^2}}$ and $\Boundb = c_2\max\Big\{ \sqrt{{\frac{p(1-p)} n}\ln\frac{e}{\regpar }}, \frac{\ln n}n,\frac{\sqrt{p(1-p)\ln n}}{\regpar n}\Big\}$, where $c_1,c_2$ are universal constants, and 
    \item $|p_S^{\tilde\AdjM}-p|\le \regpar \Boundb$.
\end{enumerate}
\end{theorem}


The subgraph over uncorrupted vertices is immune to the addition and deletion of the edges outside it, hence, from the above theorem we get the following corollary.
\begin{corollary}
For any $\corr \in [1/n,1/2)$, let $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$ and $\goodnodes$ be the set of uncorrupted nodes. Then with probability at least $1-4n^{-2}$, simultaneously for all $\regpar\in [\corr,1/2)$, subgraph over the set of uncorrupted nodes $\goodnodes$ is $(\regpar,\Bounda,\Boundb)$ regular for $\Bounda = c_1\sqrt{\frac{p(1-p)}{n}+\frac{\ln n}{n^2}}$ and $\Boundb = c_2\max\Big\{ \sqrt{{\frac{p(1-p)} n}\ln\frac{e}{\regpar }}, \frac{\ln n}n,\frac{\sqrt{p(1-p)\ln n}}{\regpar n}\Big\}$, where $c_1,c_2$ are universal constant and $|p_{\goodnodes}^{\AdjM}-p|\le \regpar \Boundb$.
\end{corollary}
In light of the above corollary, the algorithm to estimate empirical fraction of the edges of an (unknown) regular subgraph of a given graph can be applied to estimate $p$ from $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$. We will derive such an algorithm in the following subsections, but first we prove Theorem~\ref{th:erdrenyreg}.

\subsubsection{Proof of Theorem~\ref{th:erdrenyreg}}
To prove the theorem we will need the following two concentration results about randomly generated graphs using Erd\H{o}s-R\'enyi model.

The first result shows that the sum of the entries of centered version of $\tilde A$ over any of its submatrix $S\times S'$ has a small absolute value as long as each of $S$ and $S'$ either leaves out or include at most $\regpar n$ nodes.
The proof follows a Chernoff and union bound style argument, and is provided in Section~\ref{sec:app-mainconth}.
\begin{theorem}\label{th:mainconth} 
Let $\tilde A$ be the adjacency matrix of a sample from $G(n,p)$. 
There exists a universal constant $c>0$ such that with probability at least $1-3 n^{-2}$, simultaneously for all $\alpha\ge\frac{1}{n}$, we have
%and $S, S'\subseteq [n]$ such that 
%\[
%|S|, |S'|\in [0, \alpha n]\cup [n-\alpha n, n]
%\]
%we have
\[
\max_{|S|,|S'|\in \setsize_\alpha}\Big|{\langle(\tilde A-p\cdot J),J_{S\times S'}\rangle}\Big|\le c\max\Big\{ \alpha n\sqrt{{p(1-p) n}\ln\frac{e}{\alpha }},\alpha n\ln\frac{e}{\alpha },n\sqrt{p(1-p)\ln n}\Big\}.
\]
\end{theorem}

The second result bounds the spectral norm of a centered version of $\tilde A$, which follows from Remark 3.13 of~\cite{BandeiraVH16}. 
\begin{lemma}\label{lem:goodspecnormnew}
There exists a universal constant $c$ such that with probability at least $1-n^{-2}$,
$\norm{\tilde A - p\cdot J} \le c\sqrt{np(1-p)+\ln n}$.  
\end{lemma}

Using Theorem~\ref{th:mainconth}, we derive the following corollary:
\begin{corollary}
Let $\tilde A$ be the adjacency matrix of a sample from $G(n,p)$. 
There exists a universal constant $c>0$ such that with probability at least $1-3 n^{-2}$, simultaneously for all $\alpha\ge\frac{1}{n}$, and for all $S,S',S''\in C_{13\regpar}$ such that $S',S''\subseteq S$, we have
\[
\Big|{\langle(\tilde A-p_{S}^{\tilde A}\cdot J),J_{S'\times S''}\rangle}\Big|\le c\max\Big\{\alpha n\sqrt{{p(1-p) n}\ln\frac{e}{\alpha }},\alpha n\ln\frac{e}{\alpha },n\sqrt{p(1-p)\ln n}\Big\}.
\]
\end{corollary}
\begin{proof}
Note that
\begin{align*}
 \Big|{\langle(\tilde A-p_{S}^{\tilde A}\cdot J),J_{S'\times S''}\rangle}\Big|&\le \Big|{\langle(\tilde A-p\cdot J),J_{S'\times S''}\rangle}\Big|+\Big|{\langle((p_{S}^{\tilde A}-p)\cdot J),J_{S'\times S''}\rangle}\Big|.
\end{align*}
The first term on the right is bounded by Theorem~\ref{th:mainconth}. Next we bound the second term,
\begin{align*}
\Big|{\langle((p_{S}^{\tilde A}-p)\cdot J),J_{S'\times S''}\rangle}\Big|&\le \Big|{\langle((p_{S}^{\tilde A}-p)\cdot J),J_{S\times S}\rangle}\Big|\\
&=\Big|{p_{S}^{\tilde A}\cdot|S|(|S|-1)-\langle(p\cdot J),J_{S\times S}\rangle}\Big|\\
&=\Big|{\langle \tilde A,J_{S\times S}\rangle-\langle(p\cdot J),J_{S\times S}\rangle}\Big|=\Big|{\langle(\tilde A-p\cdot J),J_{S\times S}\rangle}\Big|.    
\end{align*}
Using the bound in Theorem~\ref{th:mainconth} and combing the two equations completes the proof.
\end{proof}

\begin{corollary}
There exists a universal constant $c$ such that with probability at least $1-n^{-2}$, simultaneously for all $S\subseteq[n]$, we have
$\norm{(\tilde A - p_{S}^{\tilde A}\cdot J)_{S\times S}} \le 2c\sqrt{np(1-p)+\ln n}$. 
\end{corollary}
\begin{proof}
From triangle inequality
\[
\norm{(\tilde A - p_{S}^{\tilde A}\cdot J)_{S\times S}} \le \norm{(\tilde A - p\cdot J)_{S\times S}} +\norm{((p - p_{S}^{\tilde A})\cdot J)_{S\times S}} =\norm{(\tilde A - p\cdot J)_{S\times S}} +|p - p_{S}^{\tilde A}|\cdot (|S|-1).
\]
From Lemma~\ref{lem:specnormlb} we have
\[
\norm{(\tilde A - p\cdot J)_{S\times S}}\ge \Bigg|\frac{|S|(|S|-1)p_{S}^{\tilde A}-|S|(|S|-1)p}{|S|}\Bigg|=|p - p_{S}^{\tilde A}|\cdot (|S|-1).
\]
Combining the above two equations
\[
\norm{(\tilde A - p_{S}^{\tilde A}\cdot J)_{S\times S}} \le 2\norm{(\tilde A - p\cdot J)_{S\times S}}\le 2\norm{(\tilde A - p\cdot J)}\le 2c\sqrt{np(1-p)+\ln n},
\]
where the last two inequalities use Lemma~\ref{lem:goodspecnormnew} and Lemma~\ref{lem:spsubmat}, respectively.
\end{proof}

Finally, combining the two corollaries proves the Theorem.



==> runtime.tex <==

\begin{remark}{Computational Complexity:} The spectral norm Algorithm~\ref{algo:part}, runs a total $9\gamma n$ rounds and in each round the algorithm finds the top eigenvector of an $n\times n$ matrix. However, the time required to approximate the top eigenvector of a matrix can be high if the (relative?) difference between the top two eigenvalues is small.
To avoid this we propose a simple modification to our algorithm.
In this modification, inside the while loop of algorithm~\ref{algo:part}, instead of finding the top eigenvector of $(A - p_S)_{S\times S}$, we find unit vectors $v',u'\in \mathbb R^n$ such that $(A - p_S)_{S\times S}\cdot v'>0.99\cdot ||(A - p_S)_{S\times S}||\cdot u'$, and in the next step the probability of picking an element $i\in [n]$ is $0.5(u_i'^2+v_i'^2)$.
For this proposed modification, using Corollary~\ref{cor:comp} from appendix, instead of Theorem~\ref{th:lacon}, in the proof implies the same theoretical guarantees as in Theorem~\ref{thm:specnorm}.
For any matrix $M\in\mathbb R^{n\times n}$, finding unit vectors $v',u'\in \mathbb R^n$ such that $Mv'>0.99 ||M||u'$ can be accomplished in $\mathcal O(n^2)$ time~\cite{?}, therefore, a simple modification our algorithm can be made to run in $\mathcal O(\gamma n^3)$ time.
\end{remark}

\begin{theorem}[Extention to the above theorem]
Let $M$ be a nonzero $m\times n$ real matrix such that for some sets $S_1\subseteq [m]$, $S_2\subseteq [n]$ and $0< \rho<1$ we have $\|M_{S_1\times S_2}\|\le \rho\|M\|$. 
Let $u\in \mathbb R^{ m}$ and $v\in \mathbb R^{n}$ be two unit vectors, {and $\theta \in [-1,1]$} such that $Mv = \theta \|M\| u$,
then
\[
\frac{1}{2}\Paren{\|v_{S_2^c}\|^2+\|u_{S_1^c}\|^2}\ge \frac{\theta^2 -2\rho^2}{2\max\{2(1-\rho^2 ) , \theta^2\}}.
\]
\end{theorem}
\begin{proof}
Since $Mv=\theta \|M\| u$, we have $M_{S_1\times [n]} \,v\ = \theta \|M\| u_{S_1}$, 
and furthermore, 
\begin{align*}
M_{S_1\times [n]} \,v\ = M_{S_1\times S_2}  \,v_{S_2}+ M_{S_1\times S_2^c} \,v_{S_2^c}
\end{align*}
By the triangle inequality, 
\begin{align*}
&|\theta| \cdot\|M\| \cdot\norm{u_{S_1}} \le \norm{M_{S_1\times S_2}\,v_{S_2}}+ \norm{M_{S_1\times S_2^c}\,v_{S_2^c}}\\
\Rightarrow\quad & |\theta| \cdot\|M\| \cdot\norm{u_{S_1}} \le \|M_{S_1\times S_2}\| \cdot \norm {v_{S_2}} + \|M_{S_1\times S_2^c}\| \cdot\norm{v_{S_2^c}}\\
\Rightarrow\quad & |\theta| \cdot\|M\| \cdot\norm{u_{S_1}} \le \rho \cdot\|M\| \cdot \norm {v_{S_2}} + \|M\| \cdot\norm{v_{S_2^c}}\\
\Rightarrow\quad & |\theta|\cdot \norm{u_{S_1}} \le \rho \norm {v_{S_2}} + \norm{v_{S_2^c}}\\
\Rightarrow\quad & \theta^2 \norm{u_{S_1}}^2 \le 2\rho^2 \norm {v_{S_2}}^2 +2 \norm{v_{S_2^c}}^2\\
\Rightarrow\quad & \theta^2 (1-\norm{u_{S_1^c}}^2) \le 2\rho^2 (1-\norm {v_{S_2^c}}^2) + 2\norm{v_{S_2^c}}^2\\
\Rightarrow\quad & \theta^2 -2\rho^2  \le 2(1-\rho^2 )  \norm{v_{S_2^c}}^2+ \theta^2 \norm{u_{S_1^c}}^2\\
\Rightarrow\quad & \frac{1}{2}\Paren{\|v_{S_2^c}\|^2+\|u_{S_1^c}\|^2} \ge \frac{\theta^2 -2\rho^2}{2\max\{2(1-\rho^2 ) , \theta^2\}}.
\end{align*} 
\end{proof}

\begin{corollary}\label{cor:comp}
Let $M$ be a nonzero $n\times n$ real matrix such that for some set $S\subset [n]$ and $0< \rho<1$ we have $\|M_{S\times S}\|\le \rho\|M\|$.
Let $v,u\in \mathbb R^{ n}$ be two unit vectors such that $Mv = \theta \|M\| u$, {and $\theta \in [-1,1]$}, then
$\frac{1}{2}\Paren{\|v_{S^c}\|^2+\|u_{S^c}\|^2}\ge \frac{\theta^2 -2\rho^2}{2\max\{2(1-\rho^2 ) , \theta^2\}}$. In particular, if $\rho^2\le 0.32$ and $\theta^2\ge 0.98$ then $\frac{1}{2}\Paren{\|v_{S^c}\|^2+\|u_{S^c}\|^2}\ge \frac{1}{8}$.
\end{corollary}


==> upper-bound-extreme.tex <==
In this section, we provide a method (Algorithm~\ref{algo:extreme}) for the extreme regime $p \leq 1/(n-1)$, in which the expected degree of each node is at most $1$.
\begin{theorem}\label{lem:extreme}
Let $\gamma\in [0, \frac{1}{60}]$, and $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$, for some unknown $p \leq \frac{1}{n-1}$.
Suppose that the events in Theorem~\ref{thm:extreme-conc} hold. \gnote{To add the other theorem for non-robust concentration.}
Then Algorithm~\ref{algo:extreme} returns a value $\hat p$ such that
  $|\hat p-p|\le O\left(\frac{\sqrt{p \log n}}{n} + \frac{\corr \log n}{n}\right)$ for some universal constant $c$, with probability at least $1 - \exp(-n)$ over the algorithm's random choices.
\end{theorem}

The algorithm maintains a set of heavy nodes -- those with degree much higher than one would see naturally in this extreme regime ($\Omega(\log n)$).
For each such node, we are guaranteed that it is either a corrupted node, or connected to many corrupted nodes (i.e., at least half its neighbors). 
This gives us a method for identifying corrupted nodes with reasonable probability, and by iteratively removing such nodes, we know we are done when no heavy nodes remain.

For node $i\in [n]$, let $N_i$ denote the set of neighbors of node $i$.
\begin{algorithm}[H]
  \begin{algorithmic}
    \Require{number of nodes $n$, corruption parameter $\corr\in [0, \frac1{60}]$, $\corr$-corrupted adjacency matrix $A$}
    \State{$\text{Deleted}\gets \{\}$}
    \State{$\text{HeavyNodes} \gets \{i: |N_i\setminus \text{Deleted}|\geq 2 + 18 \log n\}$}
    %\State{Comment: Namely, $S$ is the collection of nodes with degree $>c\log n$ in graph restricted to $[n]\setminus Del$.}
    \While{$|\text{HeavyNodes}|>0$}
    \State{Pick an arbitrary node $i\in \text{HeavyNodes}$}
    \State{Pick a node $j$ uniformly at random from $N_i\setminus \text{Deleted}$}
    \State{$\text{Deleted}\gets \,\text{Deleted}\cup\{i,j\}$}
    \State{$\text{HeavyNodes}\gets \{i: |N_i\setminus \text{Deleted}| \geq 2 + 18\log n\}$}
    \EndWhile\\
     \Return $p_{[n]\setminus \text{Deleted}}$ 
  \end{algorithmic}
  \caption{\label{algo:extreme} Algorithm for estimating $p$ in the extreme regime}
\end{algorithm}

To prove Theorem~\ref{lem:extreme}, we start with the following lemma.
\begin{lemma}
  \label{lem:extreme-corrupted-likely}
Let $\gamma\in [0, \frac{1}{60}]$, and $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$, for some unknown $p \leq \frac{1}{n-1}$.
Suppose that the events in Theorem~\ref{thm:extreme-conc} hold.
If during the execution of Algorithm~\ref{algo:extreme} we have $|\text{HeavyNodes}| > 0$ and thus the condition of the while loop is triggered, at least one node from the set of corrupted nodes $\bad$ is added to the set Deleted with probability at least $1/2$.
\end{lemma}
\begin{proof}
  If $i$ is a corrupted node, then we add it to Deleted and the proof is complete.
  Otherwise, by Theorem~\ref{thm:extreme-conc}, we have that the number of uncorrupted neighbors of $i$ is at most $1 + 9 \log n$. 
  Since $|N_i \setminus \text{Deleted} | > 2 + 18 \log n$, it implies that at least half of the nodes in this set must be corrupted.
  Therefore, we select a $j$ which is corrupted with probability $\geq 1/2$.
  Since $j$ is then added to Deleted, this completes the proof.
\end{proof}

To conclude the proof, we must reason about the number of edges present in the subgraph $[n] \setminus \text{Deleted}$. 
Lemma~\ref{lem:extreme-corrupted-likely}, combined with a variant of Lemma~\ref{lem:chernoff} and the fact that there are at most $\corr n$ corrupted nodes, implies that $|\text{Deleted}| \leq O(\corr n + \log n)$ with probability at least $1 - \exp(-n)$.
Prior to any corruptions, \gnote{TODO add in a lemma which says how many edges an uncorrupted subgraph of this size (which is reasonably large) has. We only use the prior sentence to reason that the subgraph is large I believe.}.
The number of edges in this subgraph is then affected only by the presence of corrupted nodes which remain in this set. 
Note that this number of nodes $|\bad \cap ([n] \setminus \text{Deleted})|$ is trivially upper bounded by $\corr n$.
When we terminate, all nodes have degree restricted to the set of nodes $[n] \setminus \text{Deleted}$ at most $2 + 18 \log n$, and thus the set of corrupted nodes can introduce at most $O(\corr n \log n)$ extra edges.
Similarly, since the events of Theorem~\ref{thm:extreme-conc} imply that the degree of any node in the original graph was at most $1 + 9 \log n$, the set of corrupted nodes could remove at most $O(\corr n \log n)$ edges.
We combine the bound on the original number of edges with these two perturbations and then rescale by the size of the subgraph to obtain Theorem~\ref{lem:extreme}.

%Since we assume the events of Theorem~\ref{thm:extreme-conc}, any node in $\goodnodes$ which is included in Deleted had at most $1 + 9 \log n$ edges in the original graph.
%Multiplying by our upper bound on the number of deleted uncorrupted nodes, by restricting our estimator to inspect only $[n] \setminus \text{Deleted}$, we neglect to count only $O(\corr n \log n + \log^2 n)$ edges which were present in the original subgraph.
%Since this in particular applies to the at most $\corr n$ corrupted nodes present, they introduce at most $O(\corr n \log n)$ extra edges.
%In particular, this bound applies to the corrupted nodes present in $[n] \setminus \text{Deleted}$, and the total amount they can perturb the number of edges present in the original subgraph is $O(\corr n + \log n)$.


==> upper-bound-spectral_old.tex <==
In this section, we propose a spectral method (Algorithm~\ref{algo:part}) with the following guarantee. We note that this result provides a \textit{coarse} estimation of $p$ with sub-optimal dependence on $\corr$. In the next section, we will post-process the result of this step to provide our near-optimal bounds. 
For this section and the following, we will assume that $\gamma \ge 1/\sqrt{n}$, which will give us optimal bounds for most regimes of interest. 

\begin{theorem}\label{lem:trimnod}
Let $\gamma\in [\frac{1}{\sqrt{n}}, \frac{1}{60}]$, and $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$, for some unknown $p$. 
Suppose that the events in Corollary~\ref{cor:goodspecnorm} hold.
Then Algorithm~\ref{algo:part} returns a subset $S^*$ such that
$|p_{S^*}-p|\le c\cdot \kappa(10\gamma,p,n) = O\left(\sqrt{\frac{p\log(1/\gamma)}{n}} +  \frac{\sqrt{\log n}}{n} + \frac{\log (1/\gamma)}{n} \right)$ for some universal constant $c$, with  probability at least $1-\exp(-\Omega(\sqrt{n}))$ over the algorithm's random choices.
\end{theorem}

%Our approach is described in Algorithm~\ref{algo:part}. It is an iterative method where at each step we remove nodes that are potentially in $B$. We maintain a set $S$ that starts with $S=[n]$. At each step we compute the top eigenvector of $(A - p_S)_{S\times S}$ and then pick a coordinate $i$ with probability $v_i^2$. We then delete $i$ from $S$ and repeat the process by $9\corr n$ times. 
\iffalse
\begin{algorithm}[H]
  \begin{algorithmic}
    \Require{$\gamma\le 1/60$, $n$, adjacency matrix $A$}
    \State{$S\gets [n]$, List $\gets\{\}$, and Del $\gets\{\}$}
    \State{List.insert$(S)$} \textit{ \ \ \ \ \ \ \ \ \ \ \ \newhz{$\triangleright$ List of all subsets $S$ along the path}}
    \While{$|\mathrm{Del}| < 9\gamma n$}
        \State{Find the top normalized eigenvector $v$ of the matrix $(A - p_S)_{S\times S}$}
        \State{$i^{D}\gets$ Randomly pick an element $i\in S$ where the probability of picking $i$ is $v_i^2$}
        \State{\newhz{$\mathrm{Del} \gets \mathrm{Del} \cup \{i^{D}\} $ and $S\gets S\setminus\{i^{D}\}$}}
        \State{List.insert$(S)$}
    \EndWhile
    \State{$S^*\gets \arg\min_{S\in \text{List}} \|(A - p_S)_{S\times S}\|$}\\
     \Return $S^*$ 
  \end{algorithmic}
  \caption{\label{algo:part}Spectral algorithm for estimating $p$}
\end{algorithm}
\fi
\begin{algorithm}[H]
  \begin{algorithmic}
    \Require{corruption parameter $\corr\in [1/\sqrt{n}, 1/60]$, adjacency matrix $A$ of $\adver(G)$}
    \State{$S\gets [n]$, Candidates $\gets\{\}$}
    \State{$\text{Candidates} \gets \text{Candidates} \cup \{S\}$} 
    \For{$t = 1$ to $9\corr n$}
        \State{Compute the top normalized eigenvector $v$ of the matrix $(A - p_S)_{S\times S}$}
        \State{Draw $i_t$ from the distribution where $i \in S$ is selected with probability $v_i^2$}
        \State{$S \gets S \setminus \{i_t\}$}
        \State{$\text{Candidates} \gets \text{Candidates} \cup \{S\}$}    \EndFor
    \State{$S^*\gets \arg\min_{S\in \text{Candidates}} \|(A - p_S)_{S\times S}\|$}\\
     \Return $S^*$ 
  \end{algorithmic}
  \caption{\label{algo:part}Spectral algorithm for estimating $p$}
\end{algorithm}

Theorem~\ref{lem:trimnod} is a consequence of the following spectral norm guarantee for Algorithm~\ref{algo:part}. 

\begin{theorem}\label{thm:specnorm}
Let $\gamma\in [\frac{1}{\sqrt{n}}, \frac{1}{60}]$, and $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$, for some unknown $p$.
Suppose that the events in Corollary~\ref{cor:goodspecnorm} hold.
Then, with  probability at least $1-\exp(-\Omega(\sqrt{n}))$, Algorithm~\ref{algo:part} returns a subset $S^*$  with \tcr{$|S^*|\ge (1-9\gamma)n$} such that $\|(A- p_{S^*})_{S^*\times S^*} \|\le 10 c_2n \cdot \kappa(10\gamma,p,n) $.
\end{theorem}

We demonstrate that Theorem~\ref{lem:trimnod} follows from Theorem~\ref{thm:specnorm}, showing that this spectral norm bound implies an estimate on the underlying parameter.
Observe that 
\begin{align}
\|(A - p_{S^*})_{S^*\times S^*}\| &\ge  \|(A-p_{S^*})_{({S^*}\cap \goodnodes)\times({S^*}\cap \goodnodes)}\| \label{eqn:noone}\\
&= \|(A-p+p-p_{S^*})_{({S^*}\cap \goodnodes)\times({S^*}\cap \goodnodes)}\|\nonumber\\
 &\ge  |p-p_{S^*}|\cdot|{S^*}\cap \goodnodes|- \|(A-p)_{({S^*}\cap \goodnodes)\times({S^*}\cap \goodnodes)}\|\label{eqn:notwo}\\
  &\ge  |p-p_{S^*}|\cdot|{S^*}\cap \goodnodes|- \|(A-p)_{ \goodnodes\times \goodnodes}\|,\label{eqn:nothree}
 \end{align}
where~\eqref{eqn:noone},~\eqref{eqn:nothree} follow from Lemma~\ref{lem:spsubmat}, and~\eqref{eqn:notwo} from Lemma~\ref{lem:triangleineq}.  Item~\ref{pt:first-point} of Corollary~\ref{cor:goodspecnorm} implies that $\|(A-p)_{ \goodnodes\times \goodnodes}\|\le cn\cdot \kappa(10\gamma,p,n)$. Combining these, 
\begin{align*}
 |p-p_{S^*}|\cdot|{S^*}\cap \goodnodes|
 &\le 10c_2n\cdot \kappa(10\gamma,p,n)+ cn\cdot \kappa(10\gamma,p,n).
\end{align*}
Using \tcr{$|S^*\cap \goodnodes|\ge |S^*|-|B|\ge (1-9\gamma)n-\gamma n\ge n/2$} yields Theorem~\ref{lem:trimnod}. 

In the remainder of this section we will prove that Algorithm~\ref{algo:part} indeed outputs a subset $S^*$ with the guarantee in Theorem~\ref{thm:specnorm}. 
The key technical argument is that if the spectral norm of $(A - p_S)_{S\times S}$ is large, then the normalized top eigenvector $v$ of $(A - p_S)_{S\times S}$ places constant weight on the subset $S \cap \bad$.
Thus, if at a given iteration Algorithm~\ref{algo:part} possesses an unsatisfactory set $S$, it will remove a corrupted node from $S \cap \bad$ with constant probability.

%satisfies $\|v_{S\cap B}\|^2\ge 0.15$, namely we select a node in $B$ with probability at least 0.15. This is formalized below.

\begin{lemma}\label{lem:delprob}
For any $\corr \in [\frac{1}{\sqrt{n}}, \frac{1}{60}]$, let $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$. 
Suppose the events in Corollary~\ref{cor:goodspecnorm} hold.
Let $S \subseteq [n]$ be of size $|S| \geq (1 - 9\corr)n$, and $v$ be the normalized top eigenvector of $(A-p_S)_{S\times S}$.
There is a universal constant $c_2$ such that if $\|(A-p_S)_{S\times S}\|\ge 10 c_2n \cdot \kappa(10\gamma,p,n) $ then $\|v_{S\cap B}\|^2\ge 0.15$.
\end{lemma}
\begin{proof}
We first require the following lemma, which lower bounds the spectral norm of a matrix $(A-p_S)_{S\times S}$ primarily in terms of the empirical estimates of $p$ corresponding the submatrices induced by $S$ and $S \cap \goodnodes$.
The proof appears in Section~\ref{sec:whatisinthename}.

\begin{lemma}\label{lem:whatisinthename}
For any $\corr \in [0,1]$, let $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$. 
For any $S \subseteq [n]$, uncorrupted set $\goodnodes \subseteq [n]$, and corrupted set $\bad = [n] \setminus \goodnodes$,
%\tcr{For any matrix $A\in \mathbb R^{n\times n}$ and $S\subseteq [n]$, and any set $\goodnodes \subset [n]$ and $B=[n]\setminus \goodnodes $,}  
\[
\|(A-p_S)_{S\times S}\|\ge  \frac{|p_{S\cap \goodnodes }-p_S|\cdot|S\cap \goodnodes |}{3}\cdot \min\left\{\sqrt{\frac{|S\cap \goodnodes |}{|S\cap B|}}, \frac{|S\cap \goodnodes |}{|S\cap B|}\right\}.
\]
\end{lemma}

For $\gamma\le 1/60$ and $|S|\ge (1-9\gamma)n$, we can deduce that $|S\cap \goodnodes|\ge n(1-10\gamma)\ge 5n/6$ and $|S\cap \bad|\le \gamma n\le n/60$. 
Therefore, ${|S\cap \bad|}/{|S\cap \goodnodes|}\le 1/50.$
By Lemma~\ref{lem:whatisinthename},
\[
|S\cap \goodnodes|\cdot|p_{S\cap \goodnodes}-p_S|\le 3\|(A-p_S)_{S\times S}\|\max\Big\{\sqrt{\frac{|S\cap B|}{|S\cap \goodnodes|}}, \frac{|S\cap B|}{|S\cap \goodnodes|}\Big\}\le \frac{3}{\sqrt{50}}\cdot \|(A-p_S)_{S\times S}\|.
\]

If $\|(A-p_S)_{S\times S}\|\ge 10 c_2n \cdot \kappa(10\gamma,p,n) $, then by  Lemma~\ref{lem:justnamed}, 
\begin{align*}
\|(A-p_S)_{(S\cap \goodnodes)\times(S\cap \goodnodes)}\|
&\le  c_2n \cdot \kappa(10\gamma,p,n)+|S\cap \goodnodes|\cdot|p_{S\cap \goodnodes}-p_S|\\
&\le \bigg(\frac{1}{10}+\frac{3}{\sqrt{50}}\bigg)\|(A-p_S)_{S\times S}\|.
\end{align*}

To interpret the above derivation: we have reasoned that if the spectral norm of $(A-p_S)_{S\times S}$ is large, the contribution due to the spectral norm of the submatrix induced by the intersection with the uncorrupted nodes $S \cap \goodnodes$ is \tcr{relatively small.} 
\tcr{This suggests that the contribution to the spectral norm by the complementary submatrix, that induced by the intersection with the corrupted nodes $S \cap \bad$, must be large.
Indeed, the following theorem formalizes this reasoning, showing that the normalized top eigenvector contains significant weight in this complementary subset of indices.
The proof appears in Section~\ref{sec:lacon}.}

%The next result states that if there exists a submatrix $M_{S\times S}$ of $M$ whose spectral norm is small relative to $\|M\|$, then the top eigenvector of $M$ must have \emph{significant mass} in $S^c=[n]\setminus S$.
% The next result will serve as a key component of our proof. It states that if a submatrix has a small norm compared to the original matrix, then the top eigenvector of the matrix must have a nontrivial weight on the complement of that subset. 
\begin{theorem}\label{th:lacon}
Let $M$ be a non-zero $n\times n$ real symmetric matrix such that for some set $S\subseteq [n]$ and $0\leq \rho\leq1$ we have $\|M_{S\times S}\|\le \rho\|M\|$. 
Let $v$ be any normalized top eigenvector of $M$.
Then
$\|v_{S^c}\|^2\ge {\frac{(1-\rho)^2}{1+(1-\rho)^2}}$.
\end{theorem}




Applying Theorem~\ref{th:lacon} with $\rho=\frac{1}{10}+\frac{3}{\sqrt{50}}$ implies that $\|v_{S\setminus (S\cap \goodnodes)}\|^2=\|v_{S\cap B}\|^2\ge \frac{(1-\rho)^2}{1+(1-\rho)^2}> 0.15$.
\end{proof}

We conclude this section with the proof of Theorem~\ref{thm:specnorm}. 

\begin{proof}[Proof of Theorem~\ref{thm:specnorm}]
It suffices to show that at least one of the sets $S$ encountered by Algorithm~\ref{algo:part} satisfies  the condition  $\|(A - p_S)_{S\times S}\|\le 10 c_2n \cdot \kappa(10\gamma,p,n)$.
From Lemma~\ref{lem:delprob} it follows that until algorithm finds such a subset $S$, the probability of deleting a corrupted node in each deletion step is at least $0.15$. 
Since there are $9 \corr n$ steps, a standard Chernoff-style argument implies that either a subset $S$ (including nodes from both $\bad$ and $\goodnodes$) satisfying the conditions of the theorem will be created, or with probability at least $1 - \exp(-\Omega(\corr n)) \geq 1 - \exp(-\Omega(\sqrt{n}))$, all nodes from $\bad$ will be deleted and thus $S \subseteq \goodnodes$.
%Therefore, if algorithm does not find such a subset $S$ {satisfying this condition} by the end of all $9\gamma n= \frac{9}{8}\cdot 8\gamma n$ deletion steps, then w.h.p. ($\approx 1-e^{-\Omega(\gamma n)}\ge 1-e^{-\Omega(\sqrt n)}$) it would delete all adversarial nodes from $S$ and hence at the end $S\subseteq \goodnodes$. 
In the latter case we apply Lemma~\ref{lem:tobenamed}, which implies that $\|(A - p_S)_{S\times S}\|\le 10 c_2n \cdot \kappa(10\gamma,p,n) $ and the theorem.
\end{proof}



\begin{remark} \tcr{Algorithm~\ref{algo:part}, runs a total $9\gamma  n$ rounds, and in each round the algorithm finds the top eigenvector of an $n\times n$ matrix. While it may be computationally expensive to find a top eigenvector, when the top eigenvalues has a small difference, as we show in Lemma~\ref{lem:comp} that finding any unit vector $v\in \mathbb R^n$ such that $|v^\intercal (A - p_S)_{S\times S} v|\le 0.99 ||(A - p_S)_{S\times S}||$ suffices. And such a unit vector can be found in $\tilde O(n^2)$ time~\cite{MuscoM15}. 
Therefore,  Algorithm~\ref{algo:part} runs in 
%$\tilde O(\gamma n^3)$ time.}
$\tilde O(\gamma n^3)$ time.}
\end{remark}


==> upper-bound-trimming-old.tex <==
In this section, we provide a trimming method (Algorithm~\ref{algo:trim}), which refines the result of Algorithm~\ref{algo:part}, improving its guarantees (quantified in Theorem~\ref{lem:trimnod}) by a factor of $\corr$.

%In this section, we will take $S^*$ the output of Algorithm~\ref{algo:part} and removes nodes from it to obtain $S^f$. We will show $p_{S^f}$, the average degree of nodes in $S^f$ has the following near-optimal guarantee. 
%{Let $S^*$ be the output of Algorithm~\ref{algo:part}. In this section, we will further remove $3\gamma n$ nodes from it to obtain $S^f$, and show that $p_{S^f}$, the average degree of nodes in $S^f$ has the following near-optimal guarantee.}
%This is a $\gamma$ factor improvement over Theorem~\ref{lem:trimnod}.
\begin{theorem}
\label{thm:main-bound}
Let $\gamma\in [\frac{1}{\sqrt{n}}, \frac{1}{60}]$, and $A$ be a $\corr$-corrupted adjacency matrix of a sample from $G(n,p)$, for some unknown $p$.
Suppose that the events in Corollary~\ref{cor:goodspecnorm} hold, and that we have some $S^*$ such that \tcr{$|S^*|\ge (1-9\gamma)n$ and} $\|(A - p_{S^*})_{S^*\times S^*}\|\le 10c_2n\cdot \kappa(10\gamma,p,n)$.
Then Algorithm~\ref{algo:trim} outputs \tcr{$p_{S^f}$} such that
%\[
%\big|p_{S^f}-p\big|\le   c_4\gamma\cdot \kappa(10\gamma,p,n)\le c_4\gamma \max\Bigg(\sqrt{\frac{p(1-p)}{n}\ln\frac{1}{\gamma}+\frac{\ln n}{n^2}} ,\frac{1}{n}\ln\frac{1}{\gamma}\Bigg).
%\]
\[
\big|p_{S^f}-p\big|\le   c_4\gamma\cdot \kappa(10\gamma,p,n) = O\left( \gamma \sqrt{\frac{p\log (1/\gamma)}{n}}+\frac{\gamma\sqrt{\log n}}{n} + \frac{\gamma\log (1/\gamma)}{n}\right).
\]
\end{theorem}

The algorithm is easy to describe. 
For $S\subseteq[n]$ and $i\in S$, we define \tcr{scores} $p_{S}^{(i)} := \frac{\sum_{j\in {S}}A_{i,j}}{|{S}|}$ to be the normalized degree of node $i$ in the subgraph induced by set $S$. 
We remove the $3\corr n$ nodes whose scores on $S^*$ deviate furthest from the average parameter $p_{S^*}$
%We remove the $3\corr n$ nodes with largest deviation from the mean $p_{S^*}$ of the entire subgraph $S^*$. 

\begin{algorithm}[H]
  \begin{algorithmic}
    \Require{number of nodes $n$, corruption parameter $\corr\in [1/\sqrt{n}, 1/60]$, $\corr$-corrupted adjacency matrix $A$, subset $S^* \subseteq [n]$}
    \State{Define the score for each node $i\in S^*$ to be $|p_{S^*}-p_{S^*}^{(i)}|$}
    \State{Remove the $3\corr n$ nodes in $S^*$ with the highest scores to obtain $S^f$}\\
     \Return \tcr{$S^f$} 
  \end{algorithmic}
  \caption{\label{algo:trim}Trimming Algorithm}
\end{algorithm}

%Throughout this section, we assume that Corollary~\ref{cor:goodspecnorm} holds, and Algorithm~\ref{algo:part} returns a subset $S^*$ such that $\|(A - p_{S^*})_{S^*\times S^*}\|\le 10c_2n\cdot \kappa(10\gamma,p,n) $ for some $c_2>0$. We have shown that these events happen with probability at least $1-4n^{-2}$. 

The first lemma shows that the average of entries of all \textit{small submatrices} of $S^*\times S^*$ are close to $p_{S^*}$.
\begin{lemma}\label{lem:somecor}
Assume the conditions of Theorem~\ref{thm:main-bound} hold.
For all $S_1,S_2\subseteq {S^*}$ with $|S_1|,|S_2|\le 3\gamma n$ we have
\begin{align*}
\Bigg|\sum_{i\in S_1,\, j\in S_2}(A_{i,j}-p_{S^*})\Bigg|\le 30c_2\gamma n^2\cdot \kappa(10\gamma,p,n).
\end{align*}
\end{lemma}
\begin{proof} Since $\|(A - p_{S^*})_{S^*\times S^*}\|\le 10c_2n\cdot \kappa(10\gamma,p,n) $, and using Lemma~\ref{lem:spsubmat} and Lemma~\ref{lem:specnormlb}, we get
%\begin{align*}
\[
\Bigg|\sum_{(i,j)\in S_1\times S_2}(A_{i,j}-p_{S^*})\Bigg|\!\le\! \sqrt{|S_1|\cdot |S_2|}\cdot \|(A-p_{S^*})_{S_1\times S_2}\| \!\le 3\gamma n\|(A-p_{S^*})_{{S^*}\times {S^*}}\|\!\le \!30c_2\gamma n^2\cdot \kappa(10\gamma,p,n).
\]\end{proof}

We now show that all the nodes in $S^{f}$ have normalized degree close to $p_{S^*}$. 
\begin{lemma}\label{lem:trimnodes}
Assume the conditions of Theorem~\ref{thm:main-bound} hold, and let $S^f$ be the output of Algorithm~\ref{algo:trim}.
There exists a universal constant $c_3>0$ such that for every node $i\in S^f$,
\[
|p_{S^*}^{(i)}-p_{S^*}|\le (2c_3+60c_2)\cdot \kappa(10\gamma,p,n).
\]
\end{lemma}
\begin{proof}
We will choose $c_3$ later. Suppose to the contrary that after $3\corr n$ nodes are deleted by Algorithm~\ref{algo:trim}, there is a node $i\in S^f$ such that $|p_{S^*}^{(i)}-p_{S^*}|> (2c_3+60c_2)\cdot \kappa(10\gamma,p,n)$. Therefore, all the nodes deleted by Algorithm~\ref{algo:trim} are such that $|p_{S^*}^{(i)}-p_{S^*}|> (2c_3+60c_2)\cdot \kappa(10\gamma,p,n)$. Let $D^+$ be the set of nodes deleted by Algorithm~\ref{algo:trim} such that $p_{S^*}^{(i)}>p_{S^*}$ for $i\in D^+$ 
and  $D^-$ be the set of deleted nodes $i$ such that $p_{S^*}^{(i)}<p_{S^*}$ for $i\in D^-$. Since $|D^+|+|D^{-}|=3\corr n$ \tcr{and $|D\setminus\goodnodes|\le |\bad|\le\gamma n$,} we have that $|D^+\cap \goodnodes|\ge \gamma n$ or $|D^-\cap \goodnodes|\ge \gamma n$. Suppose $|D^+\cap \goodnodes|\ge \gamma n$. Let $\goodnodesub=D^+\cap \goodnodes$. Then, using $|\goodnodesub|\ge\gamma n$ and $|S^*|>n/2$, we have
\begin{align*}
\sum_{i\in \goodnodesub, j\in S^*} (A_{i,j}-p_{S^*}) > |\goodnodesub|\cdot|S^*|\cdot (2c_3+60c_2)\cdot \kappa(10\gamma,p,n)\ge \gamma n^2\cdot (c_3+30c_2)\cdot \kappa(10\gamma,p,n).
\end{align*}
Now, note that 
\begin{align*}
\sum_{i\in \goodnodesub, j\in S^*} (A_{i,j}-p_{S^*}) = \sum_{i\in \goodnodesub, j\in S^*\cap \goodnodes} (A_{i,j}-{p})+ |\goodnodesub|\cdot |S^*\cap \goodnodes| \cdot (p-p_{S^*}) + \sum_{i\in \goodnodesub, j\in S^*\cap B} (A_{i,j}-p_{S^*})
\end{align*}
By Lemma~\ref{lem:somecor} with $S_1=\goodnodesub$ and $S_2=S^*\cap B$ the last term in the expression above is at most $30c_2\gamma n^2\cdot \kappa(10\gamma,p,n)$. 
For the second term note that $|p-p_{S^*}|<c \kappa(10\gamma,p,n)$ and therefore, 
the second term is at most $c\cdot \gamma n^2 \kappa(10\gamma,p,n)$. Finally invoking  Item~\ref{pt:second-point} of Corollary~\ref{cor:goodspecnorm} with $\goodnodesub$ and $\goodnodesubanother=S^*\cap \goodnodes$ and $\alpha =10\gamma$ bounds the first term by $10c_1\gamma n^2\cdot \kappa(10\gamma,p,n)$. Taking $c_3=c+10c_2$ we get the bound. The case when $|D^-\cap \goodnodes|>\gamma n$ has a similar argument and is omitted.
\end{proof}

Combining these lemmas appropriately allows us to conclude our main result on the guarantees of Algorithm~\ref{algo:trim}.
\begin{proof}[Proof of Theorem~\ref{thm:main-bound}] 
We will partition $S^f\times S^f$ into the following groups and bound each term separately. 
\begin{align*}
\sum_{i,j\in S^f}A_{i,j} = \sum_{i,j\in S^f\cap \goodnodes} A_{i,j}+  2\sum_{i\in S^f,j\in S^f\cap B} A_{i,j}-  \sum_{i,j\in S^f\cap B} A_{i,j}. 
\end{align*}
Since $p_{S^f}=\sum_{i,j\in S^f}A_{i,j}/{|S^f|^2}$, by the triangle inequality, 
\begin{align*}
\big|{p_{S^f}}-p\big|
% &=\Bigg|\frac{\sum_{i,j\in S^f}A_{i,j}}{|S^f|^2}-p\Bigg|\\
% &\le
% \Bigg|\frac{\sum_{i,j\in S^f\cap \goodnodes}(A_{i,j}-p)}{|S^f|^2}
% +2\frac{\sum_{i\in S^f  \,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}
% -\frac{\sum_{i,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|\\
&\le
\Bigg|\frac{\sum_{i,j\in S^f\cap \goodnodes}(A_{i,j}-p)}{|S^f|^2}\Bigg|
+2\Bigg|\frac{\sum_{i\in S^f  \,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|
+\Bigg|\frac{\sum_{i,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|.
\end{align*}

For the first term, $|S^f\cap \goodnodes|\ge  (1-13\gamma)n\ge n/2$. With $\goodnodesub=S^f\cap \goodnodes$ in Equation~\eqref{eq:usefula}, with $\alpha=13\corr$,
\[
{\Bigg|\frac{\sum_{i,j\in S^f\cap \goodnodes}(A_{i,j}-p)}{|S^f|^2}\Bigg|\le}\Bigg|\frac{\sum_{i,j\in S^f\cap \goodnodes}(A_{i,j}-p)}{|S^f\cap \goodnodes|^2}\Bigg| = |p_{S^f\cap \goodnodes}-p|\le 4c_1 \cdot 13\gamma\cdot \kappa(13\gamma,p,n)\le 52c_1 \gamma\cdot \kappa(10\gamma,p,n),
\]
where the last inequality uses the fact that $\kappa(\alpha,p,n)$ is a decreasing function of $\alpha$.

Since $|S^f\times (S^f\cap B)|\le \corr n^2$, by the triangle inequality, the second term is bounded by
\begin{align}
2\Bigg|\frac{\sum_{i\in S^f  \,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|
&\le 2\Bigg|\frac{\sum_{i\in S^f  \,j\in S^f\cap B}(A_{i,j}-p_{S^*})}{|S^f|^2}\Bigg| + 2\corr n^2\frac{|p_{S^*}-p|}{|S^f|^2}\nonumber\\
&\le 2\Bigg|\frac{\sum_{i\in S^*  \,j\in S^f\cap B}(A_{i,j}-p_{S^*})}{|S^f|^2}\Bigg|+2\Bigg|\frac{\sum_{i\in S^*\setminus S^f  \,j\in S^f\cap B}(A_{i,j}-p_{S^*})}{|S^f|^2}\Bigg|+8c\corr\cdot\kappa(10\corr,p,n)\nonumber.
\end{align}

Since $|S^*\setminus S^f|\le 3\corr n$ and $|S^f\cap B|\le \corr n$, by taking $S_1=S^*\setminus S^f$ and $S_2 = S^f\cap B$ in Lemma~\ref{lem:somecor} bounds the second term above by $60c_2\corr\kappa(10\corr,p,n) $. For the first term, 
\begin{align*}
\Bigg|\frac{\sum_{i\in S^*  \,j\in S^f\cap B}(A_{i,j}-p_{S^*})}{|S^f|^2}\Bigg|
&\le  \sum_{j\in S^f\cap B}\Bigg|\frac{\sum_{i\in S^*}(A_{i,j}-p_{S^*})}{n^2/4}\Bigg| \\
&\le \sum_{j\in S^f\cap B}\frac{4|S^*|}{n^2}\Bigg|\frac{\sum_{i\in S^*}(A_{i,j}-p_{S^*})}{|S^*|}\Bigg|\\
&\le \sum_{j\in S^f\cap B}\frac{4}{n}|p_j^{S^*}-p_{S^*}|\\
&\le {4}(2c_3+60c_2)\cdot \gamma\cdot\kappa(10\gamma,p,n),
\end{align*}
where we use Lemma~\ref{lem:trimnodes} and $|S^{f}\cap B|\le\gamma n$. 

For the final term, since  $|(S^f\cap B)\times (S^f\cap B)|\le \corr^2n^2$,
\begin{align*}
\Bigg|\frac{\sum_{i,j\in S^f\cap B}(A_{i,j}-p_{S^*})}{|S^f|^2}\Bigg|
&\le \Bigg|\frac{\sum_{i,j\in S^f\cap B}(A_{i,j}-p)}{|S^f|^2}\Bigg|+ |p_{S^*}-p|\cdot \frac{|S^f\cap B|^2}{|S^f|^2},
\end{align*}
which can be bounded again by taking $S_1=S_2=S^f\cap B$ in Lemma~\ref{lem:somecor}. 
\end{proof}


==> upper-prelim.tex <==


\input{concentration-properties}

